Notes on the coexistence of limit notions

We summarize the current knowledge on the three limit notions: ultrafilter-limits, closed-ultrafilter-limits and FAM-limits. Also, we consider the possibility to perform an iteration which has all the three limits and clarify the problem we face.

==> Acknowledgments.tex <==
\begin{acknowledgements}
	The author thanks his supervisor J\"{o}rg Brendle for his invaluable comments and Diego~A. Mej\'{\i}a for his helpful advice.
	This work was supported by JST SPRING, Japan Grant Number JPMJSP2148.
\end{acknowledgements}

==> Delta_system.tex <==
%%\subsection{Uniform $\Delta$-system}
%We introduce the notion of \textit{uniform $\Delta$-system}, which is a more refined $\Delta$-system of conditions in $\p^h_\gamma$ (see \cite[Definition 4.3.19.]{Uri}).
\begin{dfn}
	\label{dfn_uniform_delta_system}
	Let $\delta$ be an ordinal, 
	$h\in H$ and 
	$\bar{p}=\langle p_ m: m<\delta\rangle\in(\p_\gamma^h)^\delta$.
	$\bar{p}$ is an $h$-uniform $\Delta$-system if:
	\begin{enumerate}
		%\item There is $h\in H$ such that $p_ m\in\p_\gamma^h$ for all $ m<\delta$.
		\item $\{\dom(p_ m): m<\delta\}$ forms a $\Delta$-system with some root $\nabla$.
		\item All $|\dom(p_ m)|$ are the same $n^\prime$ and $\dom(p_ m)=\{\a_{n, m}:n<n^\prime\}$ is the increasing enumeration.
		\item There is $r^\prime\subseteq n^\prime$ such that $n\in r^\prime\Leftrightarrow\a_{n, m}\in\nabla$ for $n<n^\prime$.
		\item For $n\in n^\prime\setminus r^\prime$, $\langle\a_{n, m}: m<\delta \rangle$ is (strictly) increasing.
		
	\end{enumerate}
\end{dfn}

$\Delta$-System Lemma for this uniform $\Delta$-system also holds:
\begin{lem}(\cite[Theorem 4.3.20]{Uri})
	\label{lem_uniform_Delta_System_Lemma}
	Assume that $\theta>|H|$ is regular and $\{p_m:m<\theta\}\subseteq\bigcup_{h\in H}\p^h_\gamma$.
	Then, there exist $I\in[\theta]^\theta$ and $h\in H$ such that $\{p_m:m\in I\}$ forms an $h$-uniform $\Delta$-system.
\end{lem}
%
%\begin{proof}
%	See \cite[Theorem 4.3.20]{Uri}.
%\end{proof}

\begin{dfn}
	\label{dfn_uflimit_condition_for_iteration}
	%For $h\in H$ and $\bar{p}\in(\p^h_\gamma)^\omega$ whose domains form a $\Delta$-system with some root $\nabla$, we define $p^\infty=\lim^h\bar{p}\in\p_\gamma$ as follows:
	Let $\bar{p}=\langle p_m:m<\omega\rangle\in(\p^h_\gamma)^\omega$ be an $h$-uniform (countable) $\Delta$-system with root $\nabla$.
	We define the limit condition $p^\infty=\lim^h\bar{p}\in\p_\gamma$ as follows:
	\begin{enumerate}
		\item $\dom(p^\infty)\coloneq\nabla$.
		\item For $\xi\in\nabla$,  %$\Vdash_{\p^-_\xi}p^\infty(\xi):=\lim^{(\dot{D}^h_\xi)^-}\overline{ p(\xi)}$, where $\overline{ p(\xi)}\coloneq\langle p_m(\xi):m<\omega\rangle$.
		$\Vdash_{\p^-_\xi}p^\infty(\xi):=\lim^{(\dot{D}^h_\xi)^-}\langle p_m(\xi):m<\omega\rangle$.
\end{enumerate}
\end{dfn}




The ultrafilter limit condition forces that ultrafilter many conditions are in the generic filter:
\begin{lem}
\label{lem_UF-limit_Principle}
$\lim^h\bar{p}\Vdash_{\p_\gamma}\{m<\omega:p_m\in \dot{G}_\gamma\}\in\dot{D}^h_\gamma$.
\end{lem}



%\begin{proof}
%Induct on $\gamma$.
%
%$\textit{Successor step.}$ Let $\bar{p}=\langle(p_m,\dot{q}_m):m<\omega\rangle\in(\p^h_{\gamma+1})^\omega$ be an $h$-uniform $\Delta$-system with root $\nabla$.	
%To avoid triviality, we may assume that $\gamma\in\nabla$.
%Also we may assume that $\Vdash_{\p^-_\gamma}\dot{q}_m\in\dot{Q}_{\gamma,h(\gamma)}$ for each $m<\omega$.
%Let $p^\infty\coloneq\lim^h\langle p_m:m<\omega\rangle\in\p^-_\gamma$ and 
%$\Vdash_{\p^-_\gamma}\dot{q}^\infty\coloneq\lim^{(\dot{D}^h_\gamma)^-}\langle \dot{q}_m:m<\omega\rangle$.
%By Induction Hypothesis, $p^\infty\Vdash_{\p_\gamma}\dot{A}\coloneq\{m<\omega:p_m\in \dot{G}\}\in\dot{D}^h_\gamma$.
%By \eqref{eq_constant}, $\Vdash_{\p_\gamma}\dot{q}^\infty\Vdash_{\dot{Q}_\gamma}\dot{B}\coloneq\{m<\omega:\dot{q}_m\in \dot{H}_\gamma\}\in\dot{D}^h_{\gamma+1}$
%Thus,
%$\lim^h\bar{p}=p^\infty*\dot{q}^\infty\Vdash_{\p_{\gamma+1}}\{m<\omega:(p_m,\dot{q}_m)\in \dot{G}_\gamma*\dot{H}_\gamma\}\supseteq\dot{A}\cap\dot{B}\in \dot{D}^h_{\gamma+1}$.
%
%$\textit{Limit step.}$ Let $\gamma$ be limit and $\bar{p}=\langle p_m:m<\omega\rangle\in(\p^h_\gamma)^\omega$ be an $h$ uniform-$\Delta$-system.
%We use the same parameters as in Definition \ref{dfn_uniform_delta_system}.
%Let $\xi\coloneq\max(\nabla)+1<\gamma$ and $\bar{p}\on\xi\coloneq\langle p_m\on\xi:m<\omega\rangle$.
%Since %all $\xi_m$ are out of $\nabla$, 
%$\bar{p}\on\xi$ is also an $h$-uniform $\Delta$-system with root $\nabla$,
%$p^\infty\coloneq\lim^h\bar{p}\on\xi=\lim^h\bar{p}$.
%By Induction Hypothesis, $p^\infty\Vdash_{\p_\xi}\dot{A}\coloneq\{m<\omega:p_m\on\xi\in \dot{G}_\xi\}\in\dot{D}^h_\xi$.
%Let $n^{\prime\prime}\coloneq\max{r^\prime}+1$.
%Since $\langle \a_{n,m}:m<\omega \rangle$ is increasing for $n\in\left[n^{\prime\prime},n^\prime\right)$,
%by \eqref{eq_increasing}, 
%$\Vdash_{\p_\gamma}\dot{B}_n\coloneq\{m<\omega:p_m(\a_{n,m})\in \dot{G}_\gamma\}\in\dot{D}^h_\gamma$ for $n\in\left[n^{\prime\prime},n^\prime\right)$.
%Since $\dom(p_m)=\dom(p\on\xi)\cup\{\a_{n,m}:n\in\left[n^{\prime\prime},n^\prime\right)\}$,
%$p^\infty\Vdash_{\p_\gamma}\{m<\omega:p_m\in \dot{G}_\gamma\}=\dot{A}\cap\bigcap_{n\in\left[n^{\prime\prime},n^\prime\right)} \dot{B}_n\in \dot{D}^h_\gamma$.
%
%
%
%\end{proof}



==> Main_Lemma.tex <==
\subsection{Application to bounding-prediction}
As mentioned above,
when the first Cicho\'n's maximum was constructed in \cite{GKS}, they introduced the notion of ultrafilter-limits to keep the bounding number $\bb$ small through the iteration. This is described as follows using the notions we have already defined above:
\begin{thm}(\cite[Lemma 1.31.]{GKS})
	\label{thm_uf_limit_keeps_b_small}
	Consider the case $\Gamma=\Lambda^\mathrm{lim}_\mathrm{uf}$.
	
	Assume:
	\begin{itemize}
		\item $\kappa$ is uncountable regular and $\kappa<\gamma$.
		\item $H$ is complete and has size $<\kappa$.
	\end{itemize} 
	Then, $\p_\gamma$ forces $C_{[\gamma]^{<\kappa}}\lq \mathbf{D}$, in particular, $\bb\leq\kappa$. (Note that since a set of conditions following a common guardrail is centered, $\p_\gamma$ is $\kappa$-cc and hence preserves all cardinals $\geq\kappa$.) %In practical applications, we usually iterate ccc forcings and hence all cardinals and cofinalities are preseved.)
\end{thm}
We shall carry out a similar argument for closed-ultrafilter-limits to keep $\eeb$ small.%, using the lemmas in this subsection, which are specific for this new limit notion.

\begin{lem}
	\label{cor_UF-limit_Preservation_Property}
	Let $\bar{p}=\langle p_m :m<\omega\rangle $, $h\in H$ and $p^\infty=\lim^h\bar{p}$ as above
	and let $\varphi$ be a formula of the forcing language without parameter $m$.
	If all $p_m$ force $\varphi$, then $p^\infty$ also forces $\varphi$.
\end{lem}
\begin{proof}
	Let $G$ be any generic filter containing $p^\infty$.
	By Lemma \ref{lem_UF-limit_Principle}, in particular, there exists $p_m\in G$.
	Since $p_m$ forces $\varphi$, $V[G]\vDash\varphi$ and recall that $G$ is arbitrary containing $p^\infty$.
\end{proof}

%The following lemma is specific for $\Lambda^\mathrm{lim}_\mathrm{cuf}$ and actually this is why we consider the notion of closedness.

\begin{lem}
	\label{lem_cuf_guardrail_closedness}
	Consider the case $\Gamma=\Lambda^\mathrm{lim}_\mathrm{cuf}$.
	If $\bar{p}\in(\p^h_\gamma)^\omega$, then $\lim^h\bar{p}\in\p^h_\gamma$.
\end{lem}
\begin{proof}
	Direct from the definition of ``closed-uf-lim-linked'' in Definition \ref{dfn_UF_linked} and Definition \ref{dfn_uflimit_condition_for_iteration}.
\end{proof}




%First, we introduce some notation on the bounding-prediction.
\begin{dfn}
	%Let $Pred$ be the set of all predictors.
	For a predictor $\pi=(A,\langle \pi_k:k\in A \rangle)\in Pred$ and $f\in\oo$,
	we write $f\bpd_n \pi$ if $f(k)\leq\pi_k(f\on k)$ for all $k\geq n$ in $A$.
	Note that $\bpd=\bigcup_{n<\omega}\bpd_n $ (see Example \ref{exa_RS}) and we say $n$ is a starting point of $f\bpd\pi$ if $f\bpd_n \pi$ holds (we do not require the minimality of such $n$).
	%Let $\mathbf{BPred}$ be the relatinal system $\langle \oo, Pred, \bpd \rangle$, thus $\bb(\mathbf{BPred})=\eeb$ and $\dd(\mathbf{BPR})=\preb$.
	
\end{dfn}
%
%
%By applying the general theory of (c-)uf-limit to bounding-prediction, we can exclude a possible prediction point and preserve the information of the initial segment of predicted reals:
\begin{lem}
	\label{lem_Prediction_Point_Exclusion_Lemma}
	Let $\dot{\pi}=(\dot{A},\langle\dot{\pi}_k:k\in\dot{A}\rangle)$ be a $\p_\gamma$-name of a predictor,
	$n^*\leq j<\omega$,
	$t\in\omega^{j-1}$ and
	$\bar{p}=\langle p_m:m<\omega\rangle$ be an $h$-uniform $\Delta$-system.
	
	Assume that each $p_m$ forces:	  
	\begin{equation}
		\label{eq_PPEL_assump}
		\text{there is }c\in\oo\text{such that }c\on j=t^\frown m\text{ and }c\bpd_{n^*}\dot{\pi}.
	\end{equation}  
	Then, $\lim^h\bar{p}$ forces:
	\begin{gather}
		j-1\notin\dot{A}\text{, and}\label{eq_PPEL_conclu_1}\\
		\text{there is }c\in\oo\text{such that }c\on (j-1)=t\text{ and }c\bpd_{n^*}\dot{\pi}.\label{eq_PPEL_conclu_2}
	\end{gather}	 
\end{lem}
\begin{proof}
	Let $G$ be any generic filter containing $p^\infty\coloneq\lim^h\bar{p}$ and work in $V[G]$.
	By Lemma \ref{lem_UF-limit_Principle}, $M\coloneq\{m<\omega:p_m\in G\}\in \dot{D}^h[G]$. 
	Let $c_m\in\oo$ be a witness of \eqref{eq_PPEL_assump} for each $m\in M$.
	%	By \eqref{item_qtau_initial_segment}, 
	%	$\dot{c}_{\b_{i(\tau^\frown m)}}\on(n^*+n-1)=s^\frown\tau$ 
	%	and $\dot{c}_{\b_{i(\tau^\frown m)}}\bpd_{n^*}\dot{\pi}$ 
	%	for $m\in M_\tau$.
	
	
	If $j-1\in\dot{A}[G]$, then $c_m(j-1)=m\leq\dot{\pi}[G](c_m\on (j-1))=\dot{\pi}[G](t)$ for each $m\in M$, which contradicts that $M\in\dot{D}^h[G]$ is infinite and $\dot{\pi}[G](t)$ is a natural number.
	Thus, $j-1\notin\dot{A}[G]$ and since $G$ is arbitrary containing $p^\infty$, we obtain \eqref{eq_PPEL_conclu_1}. 
	\eqref{eq_PPEL_conclu_2} is direct from Lemma \ref{cor_UF-limit_Preservation_Property}.
	
\end{proof}
%\begin{rem}
%	This proof highlights the difference between bounding prediction and $g$-prediction for $g\in(\omega\setminus2)^\omega$ 
%	since in the case of $g$-prediction, we cannot consider such infinitely many $p_m$. Indeed, the forcing poset $\pr_g$ (defined later) has closed-ultrafilter-limits and increases $\ee_g$ and hence the limits actually do not keep $\ee_g$ small.
%	
%\end{rem}
%Lemma \ref{lem_Prediction_Point_Exclusion_Lemma} tells us one limit condition excludes one possible prediction point and preserves the information of shorter initial segments of predicted reals.
%%Let us consider the situation where there are such $\omega$-many $t$'s whose values differ only at the final point $j-2$ and we have already obtained the limit conditions $p^\infty_t$ respectively.
%%Recall that Lemma \ref{lem_cuf_guardrail_closedness}, the closedness of cUF-limits, tells us that the limit conditions are still in the position where we can again take limits of them.
%%Thus, by taking the limit of the limit conditions $p^\infty_t$'s, we can exclude the next smaller point by using shorter initial segments.
%%Also, by Corollary \ref{cor_UF-limit_Preservation_Property}, we can preserve ``$j-1\notin\dot{A}$'', the unpredictability at $j-1$, and preserve the information of the shorter initial segment. We can continue this way.
%Thus, the strategy to prove Main Lemma \ref{lem_Main_Lemma} below, which states that closed-ultrafilter-limits keep $\eeb$ small, is as follows:
%\begin{enumerate}
%	\item Assume the negation of the conclusion towards contradiction.
%	\item By a $\Delta$-system argument and arranging Cohen reals (as witnesses of $c$ in Lemma \ref{lem_Prediction_Point_Exclusion_Lemma}), satisfy the assumption of Lemma \ref{lem_Prediction_Point_Exclusion_Lemma}.
%	\item Taking limits infinitely many times (guaranteed by Lemma \ref{lem_cuf_guardrail_closedness}) in some suitable order, exclude points ``downwards'' and ultimately obtain a condition for each $j$ which excludes the points between $n^*$ and $j$.
%	\item Finally, take the limit of the ultimate conditions and exclude points ``upwards'' ($j\to\infty$), i.e., almost all points, which contradicts that there are infinitely many prediction points.
%\end{enumerate}
%

\begin{mainlem}
	\label{lem_Main_Lemma}
	Consider the case $\Gamma=\Lambda^\mathrm{lim}_\mathrm{cuf}$.
	
	Assume:
	\begin{itemize}
		\item $\kappa$ is uncountable regular and $\kappa<\gamma$.
		\item $H$ is complete and has size $<\kappa$.
	\end{itemize} 
	Then, $\p_\gamma$ forces $C_{[\gamma]^{<\kappa}}\lq \mathbf{BPR}$, in particular, $\ee\leq\eeb\leq\kappa$.
\end{mainlem}

\begin{proof}
	To avoid triviality, we may assume that each iterand is an atomless poset.
	Since $\p_\gamma$ is a fsi, we can find the first $\kappa$-many Cohen reals (as members of $\oo$) $\bar{c}\coloneq\langle \dot{c}_\b:\b<\kappa \rangle$ added at the first $\kappa$-many limit stages whose cofinalities are countable.
	For simplicity, we may assume that we have actually performed Cohen forcings in the first $\kappa$-many stages.
	We shall show that $\bar{c}$ witnesses Fact \ref{fac_Tukey_order_equivalence_condition}\eqref{item_small_equiv}, an equivalent condition of $C_{[\gamma]^{<\kappa}}\lq \mathbf{BPR}$.
	
	Assume towards contradiction that there exist a condition $p\in\p_\gamma$ and a $\p_\gamma$-name of a predictor $\dot{\pi}=(\dot{A},\langle\dot{\pi}_k:k\in\dot{A}\rangle)$ such that 
	$p\Vdash \dot{c}_\b\bpd \dot{\pi}\text{ for unboundedly many }\dot{c}_\b $.
	Let us witness the unboundedness and the starting point of the prediction $\bpd=\bigcup_{n<\omega}\bpd_n $.
	That is,
	for each $i<\kappa$ we pick $p_i\leq p$, $\b_i\in\left[i,\kappa\right)$ and $n_i<\omega$ such that $ p_i\Vdash \dot{c}_{\b_i}\bpd_{n_i}\dot{\pi}$.
	By extending and thinning, we may assume:
	
	\begin{enumerate}
		\item $\b_i\in\dom(p_i)$. (By extending $p_i$.)
		\item All $ p_i$ follow a common guardrail $h\in H$. ($|H|<\kappa$.)
		\item $\{p_i:i<\kappa\}$ forms a uniform $\Delta$-system with root $\nabla $. (By Lemma \ref{lem_uniform_Delta_System_Lemma}.)
		\item $\b_i\notin\nabla$, hence all $\b_i$ are distinct. ($\b_i$ are unbounded in $\kappa$, so $\b_i$ are eventually out of the finite set $\nabla$.)
		\item All $n_i$ are equal to $ n^*$.
		\item All $p_i(\b_i)$ are the same Cohen condition $s\in\oo$. 
		\item $|s|=n^*$. (By extending $s$ or increasing $n^*$.)
	\end{enumerate}
	
	In particular, we have that:
	\begin{equation}
		\label{eq_property_of_refined_pi}
		\text{For each }i<\kappa, p_i\text{ forces }\dot{c}_{\b_i}\on n^*=s\text{ and }\dot{c}_{\b_i}\bpd_{n^*}\dot{\pi}.
	\end{equation}
	
	Pick the first $\omega$ many $p_i$ and fix some bijection $i\colon\seq\to\omega$.
	Fix any $n<\omega$. 
	(For simplicity, we assume $n\geq3$ ).
	For each $\sigma\in\omega^n$, define $q_\sigma\leq p_{i(\sigma)}$ by extending the $\b_{i(\sigma)}$-th position $q_\sigma(\b_{i(\sigma)}):=s^\frown\sigma$.
	By \eqref{eq_property_of_refined_pi}, we have:
	\begin{equation}
		\label{eq_property_of_qtau}
		\text{For each }\sigma\in\seq, q_\sigma\text{ forces }\dot{c}_{\b_{i(\sigma)}}\on(n^*+n)=s^\frown\sigma\text{ and }\dot{c}_{\b_{i(\sigma)}}\bpd_{n^*}\dot{\pi}.
	\end{equation}
	
	
	Fix $\tau\in\omega^{n-1}$ and we consider the sequence $\bar{q}_\tau\coloneq\langle q_{\tau^\frown m}:m<\omega\rangle$.
	When defining $q_\sigma$ we changed the $\b_{i(\sigma)}$-th position which are out of $\nabla$, so $\{q_{\tau^\frown m}:m<\omega\}$ forms a uniform $\Delta$-system with root $\nabla$, following some new countable partial guardrail $h^\prime$.
	Since $H$ is complete, $h^\prime$ is extended to some $h_\tau\in H$.
	Note that 
	\begin{equation}
		\label{eq_h_h_tau_conicide}
		h_\tau\on\nabla=h^\prime\on\nabla=h\on\nabla.
	\end{equation}
	Let $q^\infty_\tau:=\lim^{h_\tau}\bar{q}_\tau $. 
	
	By Lemma \ref{lem_cuf_guardrail_closedness}, $q^\infty_\tau$ follows $h_\tau$ and by Definition \ref{dfn_uflimit_condition_for_iteration}, $\dom(q^\infty_\tau)=\nabla$.
	Thus, by \eqref{eq_h_h_tau_conicide} and Lemma \ref{lem_guarrail_folloing_only_domain}, $q^\infty_\tau$ also follows $h$.
	By \eqref{eq_property_of_qtau}, each $q_{\tau^\frown m}$ forces that:
	
	\begin{equation}
		\text{there exists }c\in\oo\text{ such that } c\on(n^*+n)=s^\frown\tau^\frown m\text{ and }c\bpd_{n^*}\dot{\pi}.
	\end{equation}
	
	Thus, we are under the assumption of Lemma \ref{lem_Prediction_Point_Exclusion_Lemma} and hence obtain:
	\begin{equation}
		q^\infty_\tau\text{ forces } n^*+n-1\notin\dot{A}\text{ and }\varphi_\tau,
	\end{equation}
	where:
	\begin{equation}
		\varphi_\tau:\equiv\text{``there exists }c\in\oo\text{ such that } c\on(n^*+n-1)=s^\frown\tau\text{ and }c\bpd_{n^*}\dot{\pi}\text{''.}
	\end{equation}
	
	Unfix $\tau$ and fix $\rho\in\omega^{n-2}$.
	We consider the sequence $\bar{q}_\rho\coloneq\langle q^\infty_{\rho^\frown m}:m<\omega\rangle$.
	Since all the domains of $q^\infty_{\rho^\frown m}$ are the same $\nabla$, 
	$\bar{q}_\rho$ is trivially a uniform $\Delta$-system with root $\nabla$.
	Also, since all $q_{\rho^\frown m}$ follow $h$, we can define $q^\infty_\rho:=\lim^h\bar{q}_\rho$.
	Similarly, we have that $\dom(q^\infty_\rho)=\nabla$ and $q^\infty_\rho$ follows $h$. 
	Note that each $q^\infty_{\rho^\frown m}$ forces $n^*+n-1\notin\dot{A}$ and $\varphi_{\rho^\frown m}$.
	Thus, we are under the assumption of Lemma \ref{lem_Prediction_Point_Exclusion_Lemma} and hence obtain that $q^\infty_\rho$ forces:
	\begin{itemize}
		\item $n^*+n-1\notin\dot{A}$.
		\item $n^*+n-2\notin\dot{A}$.
		\item $\text{there exists }c\in\oo\text{ such that }c\on(n^*+n-2)=s^\frown\rho\text{ and }c\bpd_{n^*}\dot{\pi}$.
	\end{itemize}
	(The first item is direct from Lemma \ref{cor_UF-limit_Preservation_Property}.) 
	Continuing this way, we ultimately obtain $q^n\coloneq q^\infty_\emptyset$ with the following properties:
	\begin{itemize}
		\item $\dom(q^n)=\nabla$ and $q^n$ follows $h$ (hence they form an $h$-uniform $\Delta$-system).
		\item $q^n$ forces $ \left[n^*,n^*+n\right) \cap \dot{A}=\emptyset$.
	\end{itemize}
	%(The information of the initial segments is not required anymore)
	Finally, unfix $n$ and let $q^\infty$ be the limit condition of the ultimate conditions $q^\infty:=\lim^h\langle q^n:n<\omega\rangle$.
	$q^\infty$ forces that 
	for infinitely many $n<\omega$, $\left[n^*,n^*+n\right) \cap \dot{A}=\emptyset$
	, which contradicts that $\dot{A}$ is infinite.
	
\end{proof}

%\begin{rem}
%	Roughly speaking, we first excluded points ``downwards'' and then ``upwards''. 
%	The reason for ``downwards'' is that the information of an initial segment also has that of shorter ones.
%\end{rem}

%\begin{rem}
%	The tricks of the proof are as follows:
%	\begin{itemize}
%		\item By quantifying over $c$, we succeeded to define $\varphi_\tau$ without parameter $m$ and apply Lemma \ref{lem_Prediction_Point_Exclusion_Lemma}.
%		\item By using the intervals $\left[n^*,n^*+n\right)$, we succeeded to capture the infinite set $\dot{A}$.
%	\end{itemize}
%\end{rem}


==> Q_FAM.tex <==
%\subsection{Question on FAM-limit}
\begin{que}
	In addition to Theorem \ref{thm_p_fin_prime_GCH} (Figure \ref{fig_cm_prime}), can we separate $\ee$ and $\eeb$ (and the dual numbers $\pre$ and $\preb$)?
\end{que}

In fact, even the consistency of $\max\{\ee,\bb\}<\eeb$ is not known.
We can naively define a poset $\pr^*$ which generically adds a bounding-predictor and hence increase $\eeb$, by changing the Definition \ref{dfn_PR} \eqref{item_PR_order_long} to ``$\forall n\in(d^\prime)^{-1}(\{1\})\setminus d^{-1}(\{1\}),\forall f\in F, f\on n\in\dom(\pi^\prime_n)$ and $\pi^\prime_n(f\on n)\geq f(n)$''. 
We can also show that $\pr^*$ has ultrafilter-limits by a similar proof to that of Lemma \ref{lem_pr_is_uflinked} and hence it keeps $\bb$ small. However, it is unclear whether it also keeps $\ee$ small.


\begin{que}
	\label{que_last}
	Can we additionally separate $\ee_{ubd}$ and $\nonm$ (and the dual numbers $\pre_{ubd}$ and $\covm$)?
\end{que}

This question has a deep background.

%\textit{FAM-limit} is tabled for discussion.
After the first construction of Cicho\'n's maximum in \cite{GKS}, Kellner, Shelah and T{\u{a}}nasie \cite{KST} constructed\footnote{It was constructed under the same large cardinal assumption as \cite{GKS}. Later, the assumption was eliminated in \cite{GKMS} introducing the submodel method.} Cicho\'n's maximum for another order %\footnote{Thus, all the two possible models of point-symmetrical orders were constructed at that time.} 
illustrated in Figure \ref{fig_CM_KST}, introducing the \textit{FAM-limit}\footnote{While they did not use the name ``FAM-limit'' but ``strong FAM-limit for intervals'', we use ``FAM-limit'' in this paper. %``FAM'' is short for ``finitely additive measure'' (on $\omega$). 
Also, the original idea of the notion is from \cite{She00}.} method, which focuses on (and actually is short for) finitely additive measures on $\omega$ and keeps the bounding number $\bb$ small as the ultrafilter-limit does.
\begin{figure}
	\centering
	\begin{tikzpicture}
		\tikzset{
			textnode/.style={text=black}, 
		}
		\tikzset{
			edge/.style={color=black, thin}, 
		}
		\newcommand{\w}{2.4}
		\newcommand{\h}{1.5}
		
		\node[textnode] (addN) at (0,  0) {$\addn$};
		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.25*\w, 0.5*\h) {$\theta_1$};
		
		\node[textnode] (covN) at (0,  2*\h) {$\covn$};
		\node (t3) [fill=orange, draw, text=black, circle,inner sep=1.0pt] at (0.25*\w, 1.5*\h) {$\theta_3$};
		
		
		
		\node[textnode] (addM) at (\w,  0) {$\cdot$};
		\node[textnode] (b) at (\w,  1*\h) {$\bb$};
		\node (t2) [fill=orange, draw, text=black, circle,inner sep=1.0pt] at (0.75*\w, 1.2*\h) {$\theta_2$};
		
		\node[textnode] (nonM) at (\w,  2*\h) {$\nonm$};
		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.25*\w, 2.4*\h) {$\theta_4$};
		
		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.75*\w, -0.4*\h) {$\theta_5$};
		
		\node[textnode] (d) at (\w*2,  1*\h) {$\dd$};
		\node (t7) [fill=orange, draw, text=black, circle,inner sep=1.0pt] at (2.25*\w, 0.8*\h) {$\theta_7$};
		
		\node[textnode] (cofM) at (\w*2,  2*\h) {$\cdot$};
		
		
		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
		\node (t6) [fill=orange, draw, text=black, circle,inner sep=1.0pt] at (2.75*\w, 0.5*\h) {$\theta_6$};
		
		\node[textnode] (cofN) at (\w*3,  2*\h) {$\cofn$};
		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.25*\w, 1.5*\h) {$\theta_{8}$};
		
		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
		\node[textnode] (c) at (\w*4,  2*\h) {$2^{\aleph_0}$};
		\node (tcc) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.7*\w, 2.5*\h) {$\theta_\cc$};
		
		
		
		\draw[->, edge] (addN) to (covN);
		\draw[->, edge] (addN) to (addM);
		\draw[->, edge] (covN) to (nonM);	
		\draw[->, edge] (addM) to (b);
		
		\draw[->, edge] (addM) to (covM);
		\draw[->, edge] (nonM) to (cofM);
		
		\draw[->, edge] (d) to (cofM);
		\draw[->, edge] (b) to (d);
		\draw[->, edge] (b) to (nonM);
		\draw[->, edge] (covM) to (nonN);
		\draw[->, edge] (covM) to (d);
		\draw[->, edge] (cofM) to (cofN);
		\draw[->, edge] (nonN) to (cofN);
		\draw[->, edge] (aleph1) to (addN);
		\draw[->, edge] (cofN) to (c);
		
		
		
		
		
		
		\draw[blue,thick] (-0.5*\w,1*\h)--(0.5*\w,1*\h);
		\draw[blue,thick] (2.5*\w,1*\h)--(3.5*\w,1*\h);
		
		
		\draw[blue,thick] (0.5*\w,1.5*\h)--(1.5*\w,1.5*\h);
		\draw[blue,thick] (1.5*\w,0.5*\h)--(2.5*\w,0.5*\h);
		
		
		
		\draw[blue,thick] (1.5*\w,-0.5*\h)--(1.5*\w,2.5*\h);
		%\draw[blue,thick] (0.5*\w,2.5*\h)--(0.5*\w,2.5*\h);
		\draw[blue,thick] (2.5*\w,-0.5*\h)--(2.5*\w,2.5*\h);
		
		
		\draw[blue,thick] (0.5*\w,-0.5*\h)--(0.5*\w,2.5*\h);
		%\draw[blue,thick] (2.5*\w,-0.5*\h)--(2.5*\w,0.5*\h);
		\draw[blue,thick] (-0.5*\w,-0.5*\h)--(-0.5*\w,2.5*\h);
		\draw[blue,thick] (3.5*\w,-0.5*\h)--(3.5*\w,2.5*\h);
		
		
		
		
		
		
		
		
		
	\end{tikzpicture}
	\caption{Cicho\'n's maximum constructed in \cite{KST}. Compared with the original one in \cite{GKS} (Figure \ref{fig_CM_GKS}), $\bb$ and $\covn$, $\dd$ and $\nonn$ are exchanged.} \label{fig_CM_KST}
\end{figure}

Later, Goldstern, Kellner, Mej\'{\i}a and Shelah \cite{GKMS_CM_and_evasion} proved that the FAM-limit keeps the evasion number $\ee$ small.
Recently, Uribe-Zapata formalized the theory of the FAM-limits and he, Cardona and Mej\'{\i}a generalized the result above as follows:

\begin{thmm}(\cite{Car23RIMS})
	FAM-limits keep $\non(\mathcal{E})$ small.
\end{thmm}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\tikzset{
			textnode/.style={text=black}, 
		}
		\tikzset{
			edge/.style={color=black, thin}, 
		}
		\tikzset{cross/.style={preaction={-,draw=white,line width=7pt}}}
		\newcommand{\w}{2.4}
		\newcommand{\h}{2.0}
		
		\node[textnode] (addN) at (0,  0) {$\addn$};
		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
		
		
		
		\node[textnode] (addM) at (\w,  0) {$\addm$};
		\node[textnode] (addE) at (\w,  -0.5*\h) {$\add(\mathcal{E})$};
		
		\node[textnode] (b) at (\w,  1.3*\h) {$\bb$};
		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
		
		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
		\node[textnode] (d) at (\w*2,  1.7*\h) {$\dd$};
		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cofm$};
		\node[textnode] (cofE) at (\w*2,  3.5*\h) {$\cof(\mathcal{E})$};
		
		
		
		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
		
		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
		
		\node[textnode] (e) at (0.5*\w,  1.7*\h) {$\mathfrak{e}$}; 
		\node[textnode] (pr) at (2.5*\w,  1.3*\h) {$\mathfrak{pr}$}; 
		
		\node[textnode] (estar) at (\w,  1.7*\h) {$\ee^*$};
		\node[textnode] (prstar) at (\w*2,  1.3*\h) {$\mathfrak{pr}^*$};
		
		
		\node[textnode] (eubd) at (\w*0.2,  \h*2.1) {$\ee_{ubd}$};
		\node[textnode] (prubd) at (\w*2.8,  \h*0.9) {$\mathfrak{pr}_{ubd}$};
		
		\node[textnode] (nonE) at (\w*0.75,  \h*2.55) {$\non(\mathcal{E})$};
		\node[textnode] (covE) at (\w*2.25,  \h*0.45) {$\cov(\mathcal{E})$};
		
		
		\draw[->, edge] (addM) to (nonE);
		\draw[->, edge] (covE) to (cofM);		
		\draw[->, edge] (covM) to (covE);		
		\draw[->, edge] (e) to (estar);
		\draw[->, edge] (e) to (covM);
		\draw[->, edge] (addM) to (b);
		\draw[->, edge] (e) to (estar);
		\draw[->, edge] (b) to (prstar);
		\draw[->, edge] (nonM) to (pr);
		\draw[->, edge] (prstar) to (pr);
		
		\draw[->, edge] (addN) to (covN);
		\draw[->, edge] (addN) to (addM);
		\draw[->, edge] (covN) to (nonM);	
		
		%\draw[->, edge] (b) to (nonM);
		\draw[->, edge] (addM) to (covM);
		\draw[->, edge] (nonM) to (cofM);
		%\draw[->, edge] (covM) to (d);
		\draw[->, edge] (d) to (cofM);
		
		\draw[->, edge] (covM) to (nonN);
		\draw[->, edge] (cofM) to (cofN);
		\draw[->, edge] (nonN) to (cofN);
		\draw[->, edge] (aleph1) to (addN);
		\draw[->, edge] (cofN) to (c);
		
		%\draw[->, edge] (e) to (nonM);
		
		\draw[->, edge] (addN) to (e);
		
		\draw[->, edge] (covM) to (prstar);
		
		\draw[->, edge] (pr) to (cofN);
		
		
		\draw[->, edge] (b) to (estar);C
		\draw[->, edge] (estar) to (nonM);
		\draw[->, edge] (estar) to (d);
		\draw[->, edge] (e) to (eubd);
		
		\draw[->, edge] (prstar) to (d);
		\draw[->, edge] (prstar) to (pr);
		
		
		\draw[->, edge] (prubd) to (pr);
		
		
		\draw[->, edge,cross] (eubd) to (nonE);
		\draw[->, edge] (nonE) to (nonM);
		
		\draw[->, edge] (covE) to (prubd);
		\draw[->, edge] (nonE) to (nonN);
		\draw[->, edge] (covN) to (covE);
		
		
		\draw[double distance=2pt, edge] (addM) to (addE);
		\draw[double distance=2pt, edge] (cofM) to (cofE);
		
		
		
		
		
		
		
		
		
	\end{tikzpicture}
	\caption{Cicho\'n's diagram and other cardinal invariants.}\label{fig_Cd_E}
\end{figure}
$\mathcal{E}$ denotes the $\sigma$-ideal generated by closed null sets and the four numbers related to the ideal $\mathcal{E}$ have the relationship illustrated in Figure \ref{fig_Cd_E} (Bartoszynski and Shelah \cite[Theorem 3.1]{BS92} proved $\add(\mathcal{E})=\addm$ and $\cof(\mathcal{E})=\cofm$. The other new arrows are obtained by easy observations: e.g., a $g$-predictor predicts only $F_\sigma$ null many reals and hence $\ee_{ubd}\leq\non(\mathcal{E})$ and $\cov(\mathcal{E})\leq\pre_{ubd}$ hold). Hence, FAM-limits seem to work for Question \ref{que_last} by keeping $\non(\mathcal{E})$ and $\ee_{ubd}$ small.
%Since $\non(\mathcal{E})$ is above $\ee$, FAM-limits keeps $\ee$ small.

In \cite{KST}, they also introduced the poset $\widetilde{\mathbb{E}}$ instead of $\mathbb{E}$, which increases $\nonm$ as $\mathbb{E}$ does, but has FAM-limits,  which $\mathbb{E}$ does not have. (Cardona, Mej\'{\i}a and Uribe-Zapata \cite{Car23RIMS} proved that $\mathbb{E}$ increases $\non(\mathcal{E})$ and hence does not have FAM-limits.)
Thus, if $\widetilde{\mathbb{E}}$ also had closed-ultrafilter-limits, by mixing all the three limit methods as in Theorem \ref{thm_p6fin} and \ref{thm_p_fin_prime_GCH}, it would seem to be possible to additionally separate $\ee_{ubd}$ and $\nonm$ by replacing $\mathbb{E}$ with $\widetilde{\mathbb{E}}$ through the iteration.
In fact, Goldstern, Kellner, Mej\'{\i}a and Shelah \cite{GKMS_CM_and_evasion} proved that \textit{$\widetilde{\mathbb{E}}$ actually has (closed-)ultrafilter-limits}.

%On the statement and its proof below, we use the notation introduced in \cite{KST} without the definition (see \cite{KST}).
%\begin{lem}
%	For any $t\in T^*$ and any rational number $0<\varepsilon<1$,
%	$Q=\{ p\in \dom(\loss):\trunk(p)=t\text{ and }\loss(p)\leq\varepsilon\}\subseteq\widetilde{\mathbb{E}}$ is c-uf-linked.
%	In particular, $\widetilde{\mathbb{E}}$ is $\sigma$-c-uf-lim-linked.
%\end{lem}
%
%\begin{proof}
%	Let $D$ be any ultrafilter on $\omega$.
%	We define $\lim^D\colon Q\to Q$ as follows:
%	For $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$, define $q^\infty=\lim^D\bar{q}\coloneq\{t\in T^*:X_t\in D\}$ where $X_t\coloneq\{m<\omega:t\in q_m\}$.
%	%Since $s\subseteq t$ implies $X_s\supseteq X_t$,
%	%$q^\infty$ is a subtree of $T^*$.
%	Inducting on $h<\omega$, we show:
%	\begin{equation}
%		\label{eq_Etilde_lim_lem}
%		Y_h\coloneq\{m<\omega:q^m\cap\omega^h=q^\infty\cap\omega^h\}\in D \text{ for any }h<\omega.
%	\end{equation}
%	$Y_0=\omega\in D$ trivially holds. Let $h<\omega$ and assume $Y_h\in D$.
%	Fix $s\in q^\infty\cap\omega^h$.
%	For $A\subseteq\Omega_s$,
%	define $Z_A\coloneq\{m<\omega:q_m\cap\Omega_s=A\}$.
%	Since $\bigcup\{Z_A:A\subseteq\Omega_s\}$ is a finite partition of $\omega$, there uniquely exists $A\subseteq\Omega_s$ such that $Z_A\in D$.
%	We show $A=q^\infty\cap\Omega_s$.
%	On the one hand, if $t\in A$, then $t\in q_m$ holds for any $m\in Z_A$,
%	so $Z_A\subseteq X_t$ and hence $t\in q^\infty$.
%	On the other hand, if $t\in q^\infty\cap\Omega_s$,
%	then $X_t\in D$ and we can pick some $m\in X_t\cap Z_A$.
%	$q_m$ witnesses $t\in A$.
%	Thus, $A=q^\infty\cap\Omega_s$ holds.
%	Let $W_s$ be the uniquely determined set $Z_A$ for $s\in q^\infty\cap\omega^h$.
%	Then, $Y_h\cap\bigcap\{W_s:s\in q^\infty\cap\omega^h\}\in D$ is a subset of $Y_{h+1}$ and hence the induction is done.
%	By \eqref{eq_Etilde_lim_lem}, we obtain that $q^\infty$ is a subtree of $T^*$ with the stem $t_0$,
%	$q^\infty\in\widetilde{\mathbb{E}}$ and moreover $q^\infty\in Q$ (hence the closedness of $\lim^D$ is shown).
%	To show $(\star)_n$ for $n<\omega$, let $\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega$ for $j<n$ and $r\leq\lim^D\bar{q}^j$ for all $j<n$.
%	Take $h<\omega$ larger than the length of the stem of $r$ satisfying $\pi(h)>n$ and take $t\in r\cap\omega^h$.
%	Since $t$ is also in each $\lim^D\bar{q}^j$, there exists $X\in D$ such that for all $m\in X$, $t\in q_m^j$ for all $j<n$.
%	Thus, $\leq\pi(h)$-many conditions $r$ and $\{q_m^j:j<n\}$ shares the common node $t$ above their stems, they have a common extension by Lemma 1.19. (a) in \cite{KST} where $m\in X$ is arbitrary.
%	
%	Therefore, 	$\lim^D$ witnesses $Q\subseteq\widetilde{\mathbb{E}}$ is c-D-lim-linked.
%\end{proof}

However, recall that when constructing the names of ultrafilters at limit steps in the proof of Lemma \ref{lem_uf_const_all}, we resorted to the \textit{centeredness}, which $\widetilde{\mathbb{E}}$ \textit{does not have}. %\footnote{$\widetilde{\mathbb{E}}$ is known to be between $\sigma$-linked and $\sigma$-centered: for $f,g\in\oo$ going to infinity, a poset $\p$ is $(f,g)$-linked if $\p=\bigcup_{m<\omega}\bigcap_{i>m}\bigcup_{j<f(i)}Q^i_j$ where each $Q^i_j$ is $g(i)$-linked (see e.g. \cite{OK}). Thus, $(f,g)$-linked lies between $\sigma$-linked and $\sigma$-centered (and hence it is ccc).
	%$\widetilde{\mathbb{E}}$ is proved to be $(\rho,\pi)$-linked for some (concrete) $\rho,\pi\in\oo$ (\cite[Lemma 1.19.]{KST}).}.
We have no idea on how to overcome this problem without resorting to centeredness\footnote{This is the point where Goldstern, Kellner, Mej\'{\i}a and Shelah \cite{GKMS_CM_and_evasion} found a gap in their proof, mentioned in footnote \ref{foot_MR} in Section \ref{sec_int}.\label{foot_q}}.










==> Q_UF.tex <==
%\subsection{Question on closed-ultrafilter-limit}
\begin{que}
	Are there other cardinal invariants which are not below $\eeb$ and kept small through forcings with closed-ultrafilter-limits?
\end{que}
In the left side of Cicho\'n's diagram, many cardinal invariants are either below $\eeb$ or above $\ee_{ubd}$ (hence closed-ultrafilter-limits do not keep them small) and a remaining candidate is 
$\covn$. However, not only it is unclear whether c-uf-limits keep it small, but also even if they did, it would be unclear whether there would be an application since most of the known forcings with c-uf-limits are either $\sigma$-centered or sub-random, which keep $\covn$ small without resorting to c-uf-limits.

\begin{que}
	Can the closedness argument in Main Lemma \ref{lem_Main_Lemma} be generalized to some fact such as ``closed-Fr-Knaster posets preserve strongly $\kappa$-$\mathbf{PR}^*$-unbounded families from the ground model'' described in \cite{BCM_filter_linkedness}?
\end{que}

The fact that ultrafilter limits keep $\bb$ small (Theorem \ref{thm_uf_limit_keeps_b_small}) is generalized to the fact ``For regular uncountable $\kappa$, $\kappa$-Fr-Knaster posets preserve strongly $\kappa$-$\mathbf{D}$-unbounded families from the ground model'' (\cite[Theorem 3.12.]{BCM_filter_linkedness}),
where:
\begin{itemize}
	\item Fr denotes the following linkedness notion: ``$Q\subseteq\p$ is Fr-linked if there is $\lim\colon Q^\omega\to\p$ such that $\lim\langle q_m\rangle_{m<\omega}\Vdash_\p |\{m<\omega:q_m\in\dot{G}\}|=\omega$ for any $\langle q_m\rangle_{m<\omega}\in Q^\omega$'',
	\item a $\kappa$-Fr-Knaster poset is a poset such that any family of conditions of size $\kappa$ has a Fr-linked subfamily of size $\kappa$, and
	\item a strongly $\kappa$-$\mathbf{D}$-unbounded family is a family of size $\geq\kappa$ such that any real can only dominate $<\kappa$-many reals in the family.
\end{itemize}
We are naturally interested in the possibility of this kind of generalization for closed-ultrafilter-limits. However, the proof of Main Lemma \ref{lem_Main_Lemma} basically depends on the freedom to arrange the initial segment of Cohen reals, and it seems to be hard to reflect the freedom to the reals in the ground model.





==> iteration_sufficient_condition.tex <==
We introduce a sufficient condition for ``$Q\subseteq\p$ is (c-)uf-lim-linked''. 
The condition is described in the context of pure combinatorial properties of posets and we do not have to think about forcings. 

\begin{dfn}
	\begin{itemize}
		\label{dfn_suff}
		\item Let $D$ be an ultrafilter on $\omega$, $Q\subseteq\p$ and  $\lim^D\colon Q^\omega\to\p$.
		For $n<\omega$, let $(\star)_n$ stand for:
		\begin{align*}
			(\star)_n:& \text{``Given }\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega\text{ for }j<n\text{ and }r\leq\textstyle{\lim^D}\bar{q}^j\text{ for all }j<n,\\
			&\text{then }\{m<\omega:r \text{ and all }q_m^j \text{ for } j<n \text{ have a common extension}\}\in D\text{''}.
		\end{align*}
	      
		
		
		$Q\subseteq\p$ is sufficiently-$D$-lim-linked (suff-$D$-lim-linked, for short, $Q\in\Lambda^\mathrm{suff}_D(\p)$) if there exists a function $\lim^D\colon Q^\omega\to\p$ satisfying $(\star)_n$ for all $n<\omega$.
		
%		\begin{enumerate}
%			\item \label{item_1_dfn_suff}
%			If $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$ and $r\leq\lim^D\bar{q}$,
%			then $\{m<\omega:r\text{ and }q_m \text{ are compatible}\}\in D$.
%			\item \label{item_2_dfn_suff}
%			Suppose that:
%			\begin{itemize}
%				\item $n<\omega$ and $\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega$ for $j<n$,
%				\item $r\leq\lim^D\bar{q}^j$ for all $j<n$,
%				%\item $m<\omega$ and $r$ and $q_m^j$ are compatible for all $j<n$.
%			\end{itemize}
%			Then, $\{m<\omega:r \text{ and all }q_m^j \text{ for } j<n \text{ have a common extension}\}\in D$. 
%		\end{enumerate}
		Moreover, $Q\subseteq\p$ is suff-c-$D$-lim-linked ($Q\in\Lambda^\mathrm{suff}_{\mathrm{c}D}(\p)$) if $\ran(\lim^D)\subseteq Q$.
		\item $Q\subseteq\p$ is suff-(c-)uf-lim-linked if $Q$ is $Q\subseteq\p$ is suff-(c-)$D$-lim-linked for any $D$.
		%\item $\p$ is $\mu$-suff-(c-)uf-lim-linked if $\p$ has a dense subposet which is a $\mu$-many countable union of suff-(c-)uf-lim-linked subsets.
		%As usual, when $\mu=\aleph_0$, we use ``$\sigma$'' instead.
		%\item $\Lambda^\lim_\mathrm{suff}$
	\end{itemize}
\end{dfn}

\begin{exa}
	Singletons are suff-c-uf-lim-linked and hence every poset $\p$ is $|\p|$-suff-c-uf-lim-linked.
\end{exa}

\begin{lem}
	\label{lem_suff_has_uf}
	Let $D$ be an ultrafilter on $\omega$ and $Q\subseteq\p$ is suff-$D$-lim-linked witnessed by $\lim^D$.
	Then, $Q$ is uf-lim-linked with the same witness $\lim^D$.
	In particular, $\suff\subseteq\Lambda^\mathrm{lim}_\mathrm{uf}$.
\end{lem}
\begin{proof}
	For $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$, let $\Vdash_\p \dot{A}(\bar{q})\coloneq\{m<\omega:q_m\in\dot{G}\}$.
	We show $\Vdash_\p\text{``} D\cup\{\dot{A}(\bar{q}):\bar{q}\in Q^\omega\cap V,~\lim^D\bar{q}\in\dot{G}\}$ has SFIP''.
	If not, there exist $r\in\p$, $A\in D$, $n<\omega$ and $\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega$ satisfying $r\Vdash\lim^D\bar{q}^j\in\dot{G}$ for $j<n$, 
	such that $r\Vdash A\cap\bigcap_{j<n}\dot{A}(\bar{q}^j)=\emptyset$.
	We may assume that $r\leq\lim^D\bar{q}^j$ for all $j<n$.
	%By \eqref{item_1_dfn_suff} in Definition \ref{dfn_suff}, 
	%$B^j\coloneq\{m<\omega: r\text{ and }q^j_m \text{ are compatible}\}\in D$ for each $j<n$.
	By $(\star)_n$, we can find some $m\in A$ and $\tilde{r}\leq r$ extending all $q^j_m$.
	%Since we are under the assumption of \eqref{item_2_dfn_suff} in Definition \ref{dfn_suff}, there is $\tilde{r}\leq r$ extending all $q^j_m$.
	Thus, $\tilde r\Vdash m\in A\cap\bigcap_{j<n}\dot{A}(\bar{q}^j)$, which is a contradiction.
	Hence, we can take a name of an ultrafilter $\dot{D}^\prime$ extending
	$D\cup\{\dot{A}(\bar{q}):\bar{q}\in Q^\omega\cap V,~\lim^D\bar{q}\in\dot{G}\}$.   
	Let $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$ be arbitrary.
	Since $\lim^D\bar{q}\Vdash\lim^D\bar{q}\in\dot{G}$ trivially holds,
	$\lim^D\bar{q}\Vdash\dot{A}(\bar{q})=\{m<\omega:q_m\in\dot{G}\}\in\dot{D}^\prime$ is obtained and we are done.
	
\end{proof}

%あとで　GMS引用

We show that some concrete forcing notions are $\sigma$-$\suff$-linked.
\begin{lem}(\cite{GKS})
	Eventually different forcing $\ev$ is $\sigma$-suff-c-uf-lim-linked,
	where $\ev$ is defined as follows in this paper:
	\begin{itemize}
		\item $\ev\coloneq\{(s,k,\varphi):s\in\seq, k<\omega, \varphi\colon\omega\to [\omega]^{\le k}\}$.
		\item $(s^\prime,k^\prime,\varphi^\prime)\le (s,k,\varphi)$ 
		if $s^\prime\supseteq s$, 
		$k^\prime\ge k$, $\varphi^\prime(i) \supseteq \varphi(i)$ for all $i<\omega$ and $s^\prime(i)\notin\varphi(i)$ for all $i\in\dom(s^\prime\setminus s)$.
	\end{itemize}
	
\end{lem}

\begin{proof}
	For $s\in\seq$ and $k<\omega$, let $Q_{s,k}\coloneq\{(s^\prime,k^\prime,\varphi)\in\ev:s^\prime=s,k^\prime=k\}$. We show $Q\coloneq Q_{s,k}$ is suff-c-uf-lim-linked. Let $D$ be any ultrafilter and define $\lim^D\colon Q^\omega\to Q$, $\bar{q}=\langle q_m=(s,k,\varphi_m):m<\omega\rangle\mapsto(s,k,\varphi^\infty)$ as follows:
	\[ 
	j\in \varphi_\infty(i) \Leftrightarrow \{ m<\omega: j\in \varphi_m(i)\}\in D
	\]
	We check first $(\star)_1$ and then $(\star)_n$ for $n\geq2$ ($(\star)_0$ trivially holds).
	\begin{enumerate}
		\item[$(\star)_1$:]
		Assume that $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$ and $r\leq\lim^D\bar{q}$.
		Let $r=(s^\prime,k^\prime,\varphi^\prime)$ and $\lim^D\bar{q}=(s,k,\varphi^\infty)$.
		Since $r\leq\lim^D\bar{q}$, $s^\prime(i)\notin \varphi_\infty(i)$ for all $i\in\dom(s^\prime\setminus s)$. 
		That is, $\{m<\omega:s^\prime(i)\in \varphi_m(i)\}\notin D$.
		Since $D$ is an ultrafilter, $A^i :=\{m: s^\prime(i)\notin \varphi_m(i)\}\in D$ for $i\in\dom(s^\prime\setminus s)$. 
		Let $A\coloneq\bigcap\{ A^i:i\in\dom(s^\prime\setminus s)\}\in D$ and for $m\in A$,  $s^\prime(i)\notin \varphi_m(i)$ for all $i\in\dom(s^\prime\setminus s)$. 
		Thus, $q_m$ is compatible with $r$.
		\item [$(\star)_n$:] Suppose that:
		\begin{itemize}
			\item $n\geq2$ and $\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega$ for $j<n$,
			\item $r\leq\lim^D\bar{q}^j$ for all $j<n$,
			%\item $m<\omega$ and $r$ and $q_m^j$ are compatible for all $j<n$.
		\end{itemize}
		By $(\star)_1$, $A\coloneq\bigcap_{j<n}\{m<\omega:r \text{ and }q^j_m \text{ are compatible}\}\in D$.
		Let $m\in A$ and define $r=(s^\prime,k^\prime,\varphi^\prime)$ and $q^j_m=(s,k,\varphi^j_m)$. Since $s^\prime\supseteq s$, $k^\prime\ge k$ and $r$ and $q_m^j$ are compatible,
		the condition $\tilde{r}\coloneq(s^\prime,k^\prime+nk,\tilde{\varphi})$ extends $r$ and all $q_m^j$ for $j<n$
		where $\tilde{\varphi}(i)\coloneq\varphi^\prime(i)\cup\bigcup_{j<n}\varphi^j_m(i)$ for each $i<\omega$.
		Thus, $A$ witnesses $(\star)_n$ holds.
	\end{enumerate}
	 
\end{proof}

\begin{cor}
	\label{cor_E_is_centered_suff_cuf}
	$\mathbb{E}$ is $\sigma$-$\left( \Lambda(\text{centered})\cap\Lambda^\mathrm{lim}_\mathrm{cuf}\right) $-linked.
\end{cor}
\begin{proof}
	$Q$ in the previous proof is centered and the limit function $\lim^D$ is closed in $Q$.
\end{proof}


The next example of a $\sigma$-$\Lambda^\mathrm{suff}$-linked forcing notion is \textit{$g$-prediction forcing} $\pr_g$, which generically adds a $g$-predictor and hence increases $\ee_g$, introduced in \cite{Bre95}\footnote{The name ``prediction forcing'' and the notation $\pr_g$ are not common and were not used in the original paper \cite{Bre95}, but we use the name and the notation in this paper.}.

\begin{dfn}
	\label{dfn_PR}
	Fix $g\in\left(\omega+1\setminus2\right)^\omega$.
	$g$-prediction forcing $\pr_g$ consists of tuples $(d,\pi,F)$ satisfying:
	
	\begin{enumerate}
		\item $d\in\sq$.
		\item $\pi=\langle\pi_n:n\in d^{-1}(\{1\})\rangle$.
		\item for each $n\in d^{-1}(\{1\})$, $\pi_n$ is a finite partial function of $\prod_{k<n}g(k)\to g(n)$.
		\item $F\in[\prod_{n<\omega}g(n)]^{<\omega}$
		\item for each $f,f^\prime\in F, f\on|d|=f^\prime\on|d|$ implies $f=f^\prime$.
	\end{enumerate}
	$(d^\prime,\pi^\prime,F^\prime)\leq(d,\pi,F)$ if:
	\begin{enumerate}[(i)]
		
		
		\item $d^\prime\supseteq d$.
		\item $\forall n\in d^{-1}(\{1\}), \pi_n^\prime(n)\supseteq\pi_n(n)$.
		\item $F^\prime\supseteq F$.
		\item \label{item_PR_order_long}
		$\forall n\in(d^\prime)^{-1}(\{1\})\setminus d^{-1}(\{1\}),\forall f\in F, f\on n\in\dom(\pi^\prime_n)$ and $\pi^\prime_n(f\on n)=f(n)$.
		
	\end{enumerate}
	When $g(n)=\omega$ for all $n<\omega$, we write $\pr$ instead of $\pr_g$ and just call it ``prediction forcing''.
\end{dfn}


We introduce a useful notation:
\begin{dfn}
	%Let $\zero$ be the set of all finite sequences whose values are always $0$.
	%Namely, $\zero\coloneq{0}^{<\omega}$.
	For $N<\omega$, let $\zero_N $ be the sequence of length $N$ whose values are all $0$.
	Namely, $\zero_N \coloneq N\times 1$.
	
\end{dfn}
%
%\begin{dfn}
%	Let $D$ be an ultrafilter on $\omega$ and $\bar{f}=\langle f^i\in\oo:i<\omega\rangle$. 
%	
%	If for each $n<\omega$, there (uniquely) exists $m_n\omega$ such that $\{i<\omega:f^i(n)=m_n\}$,
%	
%	we define $\bar{f}^\infty\in\oo$ by $ \bar{f}^\infty(n)=m_n$ for each $n<\omega$.
%\end{dfn}
%
%\begin{dfn}
%	Fix $k<\omega$,$d,\pi$ and $f^*=\{f^*_l\in\omega^{|d|}:l<k\}$.
%	For a countable sequence of conditions $\bar{q}=\langle p^i=(d,\pi,\{f^i_l:l<k\})\in\pr:i<\omega\rangle$ with $\forall l<k,f^i_l\on|d|=f^*_l$,
%	define:
%	\begin{itemize}
%		\item $\bar{f}_l\coloneq \langle f^i_l:i<\omega\rangle$.
%		\item $A\coloneq \{l<k:{\bar{f}_l^\infty}\text{ exists }\}, B\coloneq k\setminus A$.
%		\item $F^\infty\coloneq \{{\bar{f}_l^\infty}:l\in A\}$.
%		\item for $l\in B$, $n_l$ is the first $n<\omega$ where no $m<\omega$ satisfies $\{i<\omega:f^i_l(n)=m\}\in D$.
%		\item $n^\infty\coloneq \max\{n_l+1:l\in B\}$ (if $B=\emptyset$, $n^\infty\coloneq |d|$).
%		\item $d^\infty\coloneq d^\frown \zero_{n^\infty-|d|}\in2^{n^\infty}$.
%		\item $\lim^D\bar{q}\coloneq (d^\infty,\pi,F^\infty)$.
%	\end{itemize}
%\end{dfn}
%Note that $\lim^D{\bar{q}}$ is always defined and a condition of $\pr$.
%\begin{rem}
%	\label{rem_pr_B}
%	\item For every $l\in B$ and $m<\omega, \{i<\omega:f^i_l(n_l)>m\}\in D$.
%\end{rem}


\begin{lem}(\cite{BS_E_and_P_2})%\footnote{In \cite{BS_E_and_P_2}, Lemma \ref{lem_pr_is_uflinked} was not directly proved, but the key point of the proof of the lemma appeared there. In other words, by using the notation of this paper, the (1) part of the proof for the special case where $D$ is the cofinite filter was proved there.})
	\label{lem_pr_is_uflinked}
	$\pr_g$ is $\sigma$-centered-suff-uf-lim-linked for any $g\in\left(\omega+1\setminus2\right)^\omega$.
	If $g\in\left(\omega\setminus2\right)^\omega$, 
	then $\pr_g$ is $\sigma$-centered-c-suff-uf-lim-linked.
\end{lem}

\begin{proof}
	Fix $k<\omega$, $d,\pi$ and $f^*=\{f^*_l\in\omega^{|d|}:l<k\}$.
	Let $Q\subseteq\pr_g$ consist of every $(d^\prime,\pi^\prime,F^\prime)$
	such that $d^\prime=d, \pi^\prime=\pi$ and $F^\prime=\{f^\prime_l:l<k\})$ 
	where $f^\prime_l\on|d|=f^*_l$ for all  $l<k$.
	It is enough to show that $Q$ is centered-(c-)suff-uf-lim-linked.
	Let $D$ be any ultrafilter.
	For $\bar{f}=\langle f^i\in\oo:i<\omega\rangle$, 
	if $f^i$ satisfies that for each $n<\omega$, there (uniquely) exists $a_n<\omega$ such that $\{i<\omega:f^i(n)=a_n\}\in D$,
	we define $\bar{f}^\infty\in\oo$ by $ \bar{f}^\infty(n)=a_n$ for each $n<\omega$.
	Note that ${\bar{f}}^\infty$ is always defined if $g\in\left(\omega\setminus2\right)^\omega$.
	
	For $\bar{q}=\langle q_m=(d,\pi,\{f^m_l:l<k\})\in\pr:m<\omega\rangle\in Q^\omega$,
	define $\lim^D\bar{q}$ as follows: 
	\begin{itemize}
		\item $\bar{f}_l\coloneq\langle f^m_l:m<\omega\rangle$, $A\coloneq\{l<k:{\bar{f}_l^\infty}\text{ exists}\}, B\coloneq k\setminus A$.
		\item $F^\infty\coloneq\{{\bar{f}_l^\infty}:l\in A\}$.
		\item For $l\in B$, let $n_l$ be the first $n<\omega$ where no $a<\omega$ satisfies: 
		
		$\{m<\omega:f^m_l(n)=a\}\in D$ (hence $n_l\geq|d|$).
		\item $n^\infty\coloneq\max\{n_l+1:l\in B\}$ (if $B=\emptyset$, $n^\infty\coloneq|d|$).
		\item $d^\infty\coloneq d^\frown\zero_{n^\infty-|d|}\in2^{n^\infty}$.
		\item $\lim^D\bar{q}\coloneq(d^\infty,\pi,F^\infty)$.
	\end{itemize}
	To see $\lim^D\bar{q}$ is a condition, it is enough to show that any $f,f^\prime\in F^\infty $ with $f\on|d|=f^\prime\on|d|$ satisfies $f\on N=f^\prime\on N$ for all $N\geq|d|$. By the definition of $F^\infty$ and since $D$ is an ultrafilter, there exist $l,l^\prime\in A$ and $m<\omega$ such that $f\on N=f^m_l\on N$ and $f^\prime\on N=f^m_{l^\prime}\on N$. 
	Thus, $f\on N=f^\prime\on N$ and hence $\lim^D\bar{q}$ is a condition.
	
	Note that if $g\in\left(\omega\setminus2\right)^\omega$, then $A=k, B=\emptyset, n^\infty=|d|, d^\infty=d$ and hence $\lim^D\bar{q}\in Q$ (for any $D$).
	
	Thus, since the closedness has been shown, it is enough to show that $\lim^D$ satisfies $(\star)_n$ for $n<\omega$. We check first $(\star)_n$ for $n\geq2$ assuming $(\star)_1$ and then $(\star)_1$ since the former is easier to show.
	
	
	\begin{itemize}
		\item[$(\star)_n$:] Assuming $(\star)_1$, suppose that:
		\begin{itemize}
			\item $n\geq2$ and $\bar{q}^j=\langle q_m^j:m<\omega\rangle\in Q^\omega$ for $j<n$,
			\item $r\leq\lim^D\bar{q}^j$ for all $j<n$,
			%\item $m<\omega$ and $r$ and $q_m^j$ are compatible for all $j<n$.
		\end{itemize}
		By $(\star)_1$, $A\coloneq\bigcap_{j<n}\{m<\omega:r \text{ and }q^j_m \text{ are compatible}\}\in D$.
		Let $m\in A$ and define $r=(d^\prime,\pi^\prime,F^\prime)$ and $q^j_m=(d,\pi,F^j_m)$. Then, the condition $\tilde{r}\coloneq({d^\prime}^\frown\zero_N,\pi^\prime,F^\prime\cup\bigcup_{j<n} F^j_m)$ extends $r$ and all $q_m^j$ for $j<n$ where $N$ is large enough to satisfy 
		that any distinct functions in $F^\prime\cup\bigcup_{i<n}F_i$ have different values before $N$ (hence $\tilde{r}$ is a condition and hereafter we use ``$N$ is large enough'' in this sense).
		
		\item[$(\star)_1$:] Assume that $\bar{q}=\langle q_m:m<\omega\rangle\in Q^\omega$ and $r\leq\lim^D\bar{q}$.
		Let $r\coloneq (d^r,\pi^r,F^r)$ and $\mathrm{New}\coloneq(d^r)^{-1}(\{1\})\setminus (d^\infty)^{-1}(\{1\})$.
		
		Fix $l\in A$ and $n\in\mathrm{New}$.
		By the definition of $\bar{f}_l^\infty$,
		$ X_0\coloneq\{m<\omega: f^m_l\on(n+1)=\bar{f}_l^\infty\on(n+1)\}\in D$.
		Along with $r\leq\lim^D\bar{q}$, for $m\in X_0$, $\pi^r_n(f^m_l\on n)=\bar{f}_l^\infty(n)=f^m_l(n)$.
		
		Unfixing $l$ and $n$, we have:
		\begin{equation}
			\label{eq_pr_limit_1}
			X_1\coloneq\{m<\omega:\pi^r_n(f^m_l\on n)=f^m_l(n)\text{ for all }l\in A\text{ and } n\in\mathrm{New}\}\in D.
		\end{equation}
		Fix $l\in B$ and $n\in\mathrm{New}$.
		Let $m_n\coloneq \max\{\sigma(j):\sigma\in\dom(\pi^r_n),j<n\}$.
		Since $l\in B$, $X_2\coloneq\{m<\omega: f^m_l(n_l)>m_n\}\in D$.
		Since $n_l<n^\infty\leq n$, for all $m\in X_2, f^m_l\on n\notin\dom(\pi^r_n)$.
		Unfixing $l$ and $n$, we have:
		\begin{equation}
			\label{eq_pr_limit_2}
			X_3\coloneq\{m<\omega:f^m_l\on n\notin\dom(\pi^r_n)\text{ for all }l\in B\text{ and } n\in\mathrm{New}\}\in D.
		\end{equation}
		%By \eqref{eq_pr_limit_1} and \eqref{eq_pr_limit_2},
		It is enough to show that for all $m\in X_1\cap X_3$, $q_m$ and $r$ are compatible.
		Fix such $m$ and define (as a common extension of $q_m$ and $r$) $q^\prime\coloneq (d^\prime,\pi^\prime,F^\prime)$ as follows:
		\begin{itemize}
			\item $F^\prime\coloneq F^r\cup \{f^m_l:l<k\}$.
			\item $d^\prime=d^{r\frown} \zero_N $ where $N$ is large enough.
			\item For all $n\in (d^r)^{-1}(\{1\}), \pi^\prime_n\supseteq\pi^r_n$ and for all $l\in B$ and $n\in\mathrm{New}, \pi^\prime_n(f^m_l\on n)=f^m_l(n)$
			(This can be done by \eqref{eq_pr_limit_2}).
		\end{itemize}
		
		$q^\prime\leq r$ trivially holds since $(d^\prime)^{-1}(\{1\})\setminus (d^r)^{-1}(\{1\})=\emptyset$.
		
		To see $q^\prime\leq q_m$, we have to show:
		\begin{equation}
			\label{eq_pr_limit_3}
			\text{For all } l<k \text{ and } n\in(d^r)^{-1}(\{1\})\setminus (d)^{-1}(\{1\}), \pi^\prime_n(f^m_l\on n)=f^m_l(n).
		\end{equation}
		If $l\in A$, \eqref{eq_pr_limit_1} implies \eqref{eq_pr_limit_3}, while if $l\in B$, \eqref{eq_pr_limit_3} holds by the definition of $\pi^\prime$.
		
		
		
	\end{itemize}
	
	
\end{proof}

\begin{cor}
	\label{cor_PR_is_sigma_centered_suff}
	$\pr_g$ is $\sigma$-$\left( \Lambda(\text{centered})\cap\Lambda^\mathrm{lim}_\mathrm{uf}\right) $-linked.
	Moreover, 
	if $g\in(\omega\setminus2)^\omega$, 
	$\pr_g$ is $\sigma$-$\left( \Lambda(\text{centered})\cap\Lambda^\mathrm{lim}_\mathrm{cuf}\right)$-linked.
\end{cor}
\begin{proof}
	$Q$ in the previous proof is centered since any finitely many conditions $\{(d,\pi,F_i)\in Q:i<n\}$ have a common extension $r=(d^\frown\zero_N ,\pi,\bigcup_{i<n}F_i)$ where $N$ is large enough.
	%Also recall that the limit function is closed in $Q$ whenever $g\in(\omega\setminus2)^\omega$.
\end{proof}

















==> main_result.tex <==
\subsection{Main Results}
We\footnote{Goldstern, Kellner, Mej\'{\i}a and Shelah \cite{GKMS_CM_and_evasion} stated that they proved the same separation result, but later found a gap in their proof. Moreover, our method is different from theirs and consequently the constellation of Figure \ref{fig_thmC} is a specific separation result of ours.\label{foot_MR}} prove that the prediction and evasion numbers can be added to Cicho\'n's maximum with distinct values. %as in Figure \ref{fig_CM+e}:
%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{1.8}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.25*\w, 0.4*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  2*\h) {$\covn$};
%		\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.15*\w, 1.5*\h) {$\theta_2$};
%		
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1*\h) {$\bb$};
%		\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.6*\w, 0.7*\h) {$\theta_3$};
%		
%		\node[textnode] (e) at (0.5*\w,  1.3*\h) {$\mathfrak{e}$}; 
%		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.82*\w, 1.4*\h) {$\theta_4$};
%		
%		\node[textnode] (nonM) at (\w,  2*\h) {$\nonm$};
%		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.2*\w, 2.5*\h) {$\theta_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		\node (t6) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.8*\w, -0.5*\h) {$\theta_6$};
%		
%		\node[textnode] (pr) at (2.5*\w,  0.7*\h) {$\mathfrak{pr}$}; 
%		\node (t7) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.18*\w, 0.6*\h) {$\theta_7$};
%		
%		\node[textnode] (d) at (\w*2,  1*\h) {$\dd$};
%		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.4*\w, 1.3*\h) {$\theta_8$};
%		
%		\node[textnode] (cofM) at (\w*2,  2*\h) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.85*\w, 0.5*\h) {$\theta_9$};
%		
%		\node[textnode] (cofN) at (\w*3,  2*\h) {$\cofn$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.25*\w, 1.6*\h) {$\theta_{10}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  2*\h) {$2^{\aleph_0}$};
%		\node (tcc) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.7*\w, 2.5*\h) {$\theta_\cc$};
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (d);
%		\draw[->, edge] (b) to (nonM);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (covM) to (d);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		\draw[->, edge] (e) to (nonM);
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		\draw[->, edge] (covM) to (pr);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (pr) to (cofN);
%		
%		
%		
%		
%		
%		\draw[blue,thick] (-0.5*\w,1*\h)--(0.35*\w,1*\h);
%		\draw[blue,thick] (2.65*\w,1*\h)--(3.5*\w,1*\h);
%		
%		
%		\draw[blue,thick] (0.35*\w,1.65*\h)--(1.5*\w,1.65*\h);
%		\draw[blue,thick] (1.5*\w,0.35*\h)--(2.65*\w,0.35*\h);
%		
%		\draw[blue,thick] (0.35*\w,1.15*\h)--(1.5*\w,1.15*\h);
%		\draw[blue,thick] (1.5*\w,0.85*\h)--(2.65*\w,0.85*\h);
%		
%		
%		
%		\draw[blue,thick] (1.5*\w,-0.5*\h)--(1.5*\w,2.5*\h);
%		%\draw[blue,thick] (0.5*\w,2.5*\h)--(0.5*\w,2.5*\h);
%		\draw[blue,thick] (2.65*\w,-0.5*\h)--(2.65*\w,2.5*\h);
%		
%		
%		\draw[blue,thick] (0.35*\w,-0.5*\h)--(0.35*\w,2.5*\h);
%		%\draw[blue,thick] (2.5*\w,-0.5*\h)--(2.5*\w,0.5*\h);
%		\draw[blue,thick] (-0.5*\w,-0.5*\h)--(-0.5*\w,2.5*\h);
%		\draw[blue,thick] (3.5*\w,-0.5*\h)--(3.5*\w,2.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Cicho\'n's maximum with evasion/prediction numbers.}\label{fig_CM+e}
%\end{figure}

\begin{thmA}(Theorem \ref{thm_p6fin})
	\label{thmA}
	$\aleph_1<\addn<\covn<\bb<\ee<\nonm<\covm<\pre<\dd<\nonn<\cofn<2^{\aleph_0}$ consistently holds. %where $\aleph_1\leq\theta_1\leq\cdots\leq\theta_{10}$ are regular and $\theta_\cc\geq\theta_{10}$ satisfies $\theta_\cc^{\aleph_0}=\theta_\cc$.
\end{thmA}

%Let us review the history of Cicho\'n's maximum focusing on the methods.
The construction of Cicho\'n's maximum consists of two steps: the first one is to separate the left side of the diagram with additional properties and the second one is to separate the right side (point-symmetrically) using these properties. In \cite{GKS}, the large cardinal assumption was used in the second step to apply \textit{Boolean Ultrapowers}. In \cite{GKMS}, they introduced the \textit{submodel} method instead, which is a general technique to separate the right side without large cardinals.

Let us focus on the first step. The main work to separate the left side is \textit{to keep the bounding number $\bb$ small} through the forcing iteration, since the naive bookkeeping iteration to increase the cardinal invariants in the left side guarantees the smallness of the other numbers but not of $\bb$.
To tackle the problem, in \cite{GKS} they used the \textit{ultrafilter-limit} %\footnote{While they did not use the name ``ultrafilter-limit'' but ``$\lim^D$'' for an ultrafilter $D$ on $\omega$, we use ``ultrafilter-limit'' in this paper.}
method, which was first introduced by Goldstern, Mej\'{\i}a and Shelah \cite{GMS16} to separate the left side of the diagram. 
%and in \cite{KST} they introduced the \textit{FAM-limit}\footnote{While they did not use the name ``FAM-limit'' but ``strong FAM-limit for intervals'', we use ``FAM-limit'' in this paper. ``FAM'' is short for ``finitely additive measure'' (on $\omega$). Also, the original idea of the notion is seen in \cite{She00}} method.


We introduce a new limit method called \textit{closed-ultrafilter-limit} (Definition \ref{dfn_UF_linked}), which is a variant of ultrafilter-limit, and prove that it keeps $\ee$ small:
\begin{thmB}(Main Lemma \ref{lem_Main_Lemma})
	Closed-ultrafilter-limits keep $\ee$ small.
\end{thmB}
We also prove that the two ultrafilter-limit methods can be mixed and obtain a new separation model (Theorem A, Theorem \ref{thm_p6fin}).

Moreover, we prove that we can control the values of the following variants of the evasion/prediction numbers:


\begin{dfn}
	\label{dfn_variant}
	\begin{enumerate}
		\item A predictor $\pi$ \textit{bounding-predicts} $f\in\oo$ if $f(n)\leq\pi(f\on n)$ for all but finitely many $n\in D$.
		$\preb$ and $\eeb$ denote the prediction/evasion number respectively with respect to the bounding-prediction.
		\item Let $g\in\left(\omega+1\setminus2\right)^\omega$. ( ``$\setminus2$'' is required to exclude trivial cases.)
	%	\begin{itemize}
			%\item 
			\textit{$g$-prediction} is the prediction where the range of functions $f$ is restricted to $\prod_{n<\omega}g(n)$ and $\pre_g$ and $\ee_g$ denote the prediction/evasion number respectively with respect to the $g$-prediction.
			Namely,
			\begin{gather*}
				\mathfrak{pr}_g\coloneq\min\{|\Pi|:\Pi\subseteq Pred,\forall f\in\textstyle{\prod_{n<\omega}g(n)}~\exists\pi\in \Pi~\pi \text{ predicts } f\},\\
				\mathfrak{e}_g\coloneq\min\{|F|:F\subseteq\textstyle{\prod_{n<\omega}g(n)},\forall \pi\in Pred~\exists f\in F~ f\text{ evades }\pi\}.
			\end{gather*}
			Define:
			\begin{gather*}
				\mathfrak{pr}_{ubd}\coloneq\sup\left\{\mathfrak{pr}_g:g\in\left(\omega\setminus2\right)^\omega\right\},\\
				\ee_{ubd}\coloneq\min\left\{\ee_g:g\in\left(\omega\setminus2\right)^\omega\right\}.
			\end{gather*}
			
	
	\end{enumerate}
	
\end{dfn}

%The new numbers can be embedded into the diagram as in Figure \ref{fig_Cd_all}. 
We obtain the following separation result:
\begin{thmC}(Theorem \ref{thm_p_fin_prime_GCH})
	\label{thmC}
	$\aleph_1<\addn<\covn<\bb<\ee=\eeb<\ee_{ubd}=\nonm<\covm=\pre_{ubd}<\preb=\pre<\dd<\nonn<\cofn<2^{\aleph_0}$ consistently holds.
\end{thmC}

%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{2.0}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		%\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.25*\w, 0.8*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		%\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.15*\w, 3.3*\h) {$\theta_2$};
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1.3*\h) {$\bb$};
%		%\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.68*\w, 1.2*\h) {$\theta_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		%\node (t7) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.65*\w, -0.3*\h) {$\theta_7$};
%		
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		
%		\node[textnode] (d) at (\w*2,  1.7*\h) {$\dd$};
%		%\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.32*\w, 1.8*\h) {$\theta_{10}$};
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		%\node (t11) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.85*\w, -0.3*\h) {$\theta_{11}$};
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		%\node (t12) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.25*\w, 2.2*\h) {$\theta_{12}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		%\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.67*\w, 3.4*\h) {$\theta_\cc$};
%		
%		\node[textnode] (e) at (0.5*\w,  1.7*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  1.7*\h) {$\ee^*$};
%		%\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.15*\w, 1.7*\h) {$\theta_4$};
%		
%		
%		\node[textnode] (pr) at (2.5*\w,  1.3*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1.3*\h) {$\mathfrak{pr}^*$};
%		%\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.85*\w, 1.3*\h) {$\theta_9$};
%		
%		\node[textnode] (eubd) at (\w*0.75,  \h*2.45) {$\ee_{ubd}$};
%		%\node[textnode] (nonE) at (\w*0.75,  \h*2.55) {$\non(\mathcal{E})$};
%		%\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.5*\w, 2.1*\h) {$\theta_5$};%0.5 2.1
%		
%		\node[textnode] (prubd) at (\w*2.25,  \h*0.55) {$\mathfrak{pr}_{ubd}$};
%		%\node[textnode] (covE) at (\w*2.25,  \h*0.45) {$\cov(\mathcal{E})$};
%		%\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.47*\w, 0.9*\h) {$\theta_8$};
%		
%		
%		
%		
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		%\draw[->, edge] (b) to (nonM);
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		%\draw[->, edge] (covM) to (d);
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		%\draw[->, edge] (e) to (nonM);
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (covM) to (prubd);
%		\draw[->, edge] (covN) to (prubd);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);C
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (estar) to (d);
%		\draw[->, edge] (e) to (eubd);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		\draw[->, edge] (prubd) to (pr);
%		\draw[->, edge] (eubd) to (nonM);
%		\draw[->, edge] (eubd) to (nonN);
%
%		
%		
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Cicho\'n's diagram with the variants of evasion/prediction numbers.}\label{fig_Cd_all}
%\end{figure}
%%
%%
%%
%%
%%
%%
%%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{2.0}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.2*\w, 0.8*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.15*\w, 2.45*\h) {$\theta_2$};
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1.3*\h) {$\bb$};
%		\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.68*\w, 1.2*\h) {$\theta_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.0*\w, 3.3*\h) {$\theta_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		\node (t6) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.0*\w, -0.3*\h) {$\theta_6$};
%		
%		\node[textnode] (d) at (\w*2,  1.7*\h) {$\dd$};
%		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.32*\w, 1.8*\h) {$\theta_{8}$};
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.85*\w, 0.55*\h) {$\theta_{9}$};
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.25*\w, 2.2*\h) {$\theta_{10}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.67*\w, 3.4*\h) {$\theta_\cc$};
%		
%		\node[textnode] (e) at (0.5*\w,  1.7*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  1.7*\h) {$\ee^*$};
%		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.75*\w, 1.9*\h) {$\theta_4$};
%		
%		
%		\node[textnode] (pr) at (2.5*\w,  1.3*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1.3*\h) {$\mathfrak{pr}^*$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.25*\w, 1.1*\h) {$\theta_7$};
%		
%		\node[textnode] (eubd) at (\w*0.75,  \h*2.45) {$\ee_{ubd}$};
%		%\node[textnode] (nonE) at (\w*0.75,  \h*2.55) {$\non(\mathcal{E})$};
%		%\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.5*\w, 2.1*\h) {$\theta_5$};%0.5 2.1
%		
%		\node[textnode] (prubd) at (\w*2.25,  \h*0.55) {$\mathfrak{pr}_{ubd}$};
%		%\node[textnode] (covE) at (\w*2.25,  \h*0.45) {$\cov(\mathcal{E})$};
%		%\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.47*\w, 0.9*\h) {$\theta_8$};
%		
%		
%		
%		
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		%\draw[->, edge] (b) to (nonM);
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		%\draw[->, edge] (covM) to (d);
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		%\draw[->, edge] (e) to (nonM);
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (covM) to (prubd);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (covN) to (prubd);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);C
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (eubd) to (nonN);
%		\draw[->, edge] (estar) to (d);
%		\draw[->, edge] (e) to (eubd);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		\draw[->, edge] (prubd) to (pr);
%		\draw[->, edge] (eubd) to (nonM);
%		%		\
%		%		
%		%		\draw[->, edge] (eubd) to (nonE);
%		%		\draw[->, edge] (addM) to (nonE);
%		%		\draw[->, edge] (nonE) to (nonM);
%		%		
%		%		\draw[->, edge] (covE) to (prubd);
%		%		\draw[->, edge] (covE) to (cofM);
%		%		\draw[->, edge] (covM) to (covE);
%		
%		\draw[blue,thick] (-0.5*\w,1.5*\h)--(3.5*\w,1.5*\h);
%		\draw[blue,thick] (1.5*\w,-0.5*\h)--(1.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (-0.5*\w,-0.5*\h)--(-0.5*\w,3.5*\h);
%		\draw[blue,thick] (3.5*\w,-0.5*\h)--(3.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (0.5*\w,-0.5*\h)--(0.5*\w,1.5*\h);
%		\draw[blue,thick] (2.5*\w,1.5*\h)--(2.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (0.3*\w,2.25*\h)--(1.5*\w,2.25*\h);
%		%\draw[blue,thick] (-0.3*\w,2.7*\h)--(1.5*\w,2.7*\h);
%		\draw[blue,thick] (0.3*\w,1.5*\h)--(0.3*\w,2.25*\h);
%		\draw[blue,thick] (0.5*\w,2.25*\h)--(0.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (2.7*\w,0.8*\h)--(1.5*\w,0.8*\h);
%		%\draw[blue,thick] (3.1*\w,0.3*\h)--(1.5*\w,0.3*\h);
%		\draw[blue,thick] (2.7*\w,1.5*\h)--(2.7*\w,0.8*\h);
%		\draw[blue,thick] (2.5*\w,0.8*\h)--(2.5*\w,-0.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Separation constellation of Theorem C.}\label{fig_thmC}
%\end{figure}




==> modi_separation.tex <==
\subsection{Separation of the left side}
\newcommand{\ind}{i}
\newcommand{\pst}{\mathbb{P}}
We are ready to prove the main theorem, \textit{Cicho\'n's maximum with evasion number}. %We roughly follow the flow of the original construction of Cicho\'n's maximum in \cite{GKS} and \cite{GKMS}, i.e., we first separate the left side of the diagram by performing a fsi %like \cite{GKS}
%and then the right side by submodel method introduced in \cite{GKMS}.
%However, there is a problem that the cardinal arithmetics we shall assume for the separation of the left (Assumption \ref{ass_for_complete_guardrail}) and that of the right (GCH\footnote{While we can actually weaken the assumption more than GCH, but we assume GCH in this paper for simplicity. See \cite{forcing_constellations} for details.}) actually \textit{conflicts}.
%To overcome this problem, we construct three posets $\pst_{\mathrm{pre}}$, $\pst_{\mathrm{mid}}$ and $\pst_{\mathrm{fin}}$ in this order:
%First, we construct $\pst_{\mathrm{pre}}$ which separates the left side under the cardinal arithmetic Assumption \ref{ass_for_complete_guardrail}.
%Then, we construct under GCH $\pst_{\mathrm{mid}}$ whose separation constellation is the same as $\pst_{\mathrm{pre}}$'s, by mimicking the construction of $\pst_{\mathrm{pre}}$ (This kind of argument of recovering GCH originally appears in \cite{GKS}).
%Finally, we construct $\pst_{\mathrm{fin}}$ which separates also the right side by using the submodel method using GCH.


\begin{dfn}
	\begin{itemize}
		\item $\R_1\coloneq\mathbf{Lc}^*$ and $\br_1\coloneq\mathbb{A}$, the Amoeba forcing.
		\item $\R_2\coloneq\mathbf{Cn}$ and $\br_2\coloneq\mathbb{B}$, the random forcing.
		\item $\R_3\coloneq\mathbf{D}$ and $\br_3\coloneq\mathbb{D}$, the Hechler forcing.
		\item $\R_4\coloneq\mathbf{PR}$, $\R_4^*\coloneq\mathbf{BPR}$ and $\br_4\coloneq\mathbb{PR}$.
		\item $\R_5\coloneq\mathbf{Mg}$ and $\br_5\coloneq\mathbb{E}$.
	\end{itemize}
	Let $I\coloneq\{1,\ldots,5\}$ be the index set.
\end{dfn}
Hence, $\br_{\ind}$ is the poset which increases $\bb(\R_\ind)$ for each $\ind\in I$.
Also note that $\R_4^*\lq\R_4$.
\begin{ass}
	\label{ass_card_arith}
	
	\begin{enumerate}
		\item $\lambda_1<\cdots<\lambda_6$ are regular uncountable cardinals.
		\item $\lambda_3=\mu_3^+$ and $\lambda_4=\mu_4^+$ are successor cardinals and $\mu_3$ is regular.
		\item \label{item_aleph1_inacc}$\kappa<\lambda_\ind$ implies $\kappa^{\aleph_0}<\lambda_\ind$ for all $\ind\in I$.
		%\item $\lambda_3^{\aleph_0}<\lambda_4$ and $\lambda_4^{\aleph_0}<\lambda_5$.
		\item \label{item_ca_3}
		$\lambda_6^{<\lambda_5}=\lambda_6$, hence $\lambda_6^{<\lambda_\ind}=\lambda_6$ for all $\ind\in I$.
		
		
	\end{enumerate}
\end{ass}

\begin{lem}
	\label{lem_ccc_rs}
	Every ccc poset forces $C_{[\lambda_6]^{<\lambda_\ind}}\cong_T C_{[\lambda_6]^{<\lambda_\ind}}\cap V\cong_T[\lambda_6]^{<\lambda_\ind}\cap V\cong_T[\lambda_6]^{<\lambda_\ind}$ for any $\ind\in I$.
\end{lem}

\begin{proof}
	Direct from Fact \ref{fac_suff_eq_CI_and_I}, Fact \ref{fac_cap_V} and Assumption \ref{ass_card_arith} \eqref{item_ca_3}.
\end{proof}

Thus, we often identify the four relational systems in Lemma \ref{lem_ccc_rs} in this section.

\begin{dfn}
	Put $\gamma\coloneq\lambda_6$, the length of the iteration we shall perform. Fix $S_1\cup\cdots\cup S_5=\gamma$, a cofinal partition of $\lambda_6$ and for $\xi<\gamma$, let $\ind(\xi)$ denote the unique $\ind\in I$ such that $\xi\in S_\ind$.
\end{dfn}

We additionally assume the following cardinal arithmetic to obtain a complete set of guardrails.
\begin{ass}
	\label{ass_for_complete_guardrail}
	$\lambda_6\leq2^{\mu_3}$.
\end{ass}
%Note that this Assumption \ref{ass_for_complete_guardrail} conflicts with GCH.






\begin{lem}
	There exist complete sets $H$ and $H^\prime$ of guardrails of length $\gamma=\lambda_6$ for $\lambda_3$-$\Lambda^\mathrm{lim}_\mathrm{uf}$-iteration of size $<\lambda_3$ and $\lambda_4$-$\Lambda^\mathrm{lim}_\mathrm{cuf}$-iteration of size $<\lambda_4$, respectively.  
\end{lem}

\begin{proof}
	Direct from Lemma \ref{cor_complete}, Assumption \ref{ass_card_arith} \eqref{item_aleph1_inacc} and \ref{ass_for_complete_guardrail}.
\end{proof}


By the lemmas we have proved, we can perform the iteration below (see \cite{Yam24} for details).
\begin{con}
	\label{con_P6}
	We can construct a ccc finite support iteration $\pst_\mathrm{pre}$ satisfying the following items:
	\begin{enumerate}
		\item \label{item_P6_1}
		$\pst_\mathrm{pre}$ is a $\lambda_3$-$\Lambda^\mathrm{lim}_\mathrm{uf}$-iteration of length $\gamma\coloneq\lambda_6$ and has $\Lambda^\mathrm{lim}_\mathrm{uf}$-limits on $H$ 
		with the following witnesses:
		\begin{itemize}
			\item $\langle\p_\xi^-:\xi<\gamma\rangle$, the complete subposets witnessing $\Lambda^\mathrm{lim}_\mathrm{uf}$-linkedness.
			\item $\bar{Q}=\langle\dot{Q}_{\xi,\zeta}:\zeta<\theta_\xi,\xi<\gamma\rangle$, the $\Lambda^\mathrm{lim}_\mathrm{uf}$-linked components.
			\item $\bar{D}=\langle \dot{D}^h_\xi:\xi\leq\gamma,~h\in H \rangle$, the ultrafilters.
			\item $S^-\coloneq S_1\cup S_2\cup S_3$, the trivial stages and $S^+\coloneq S_4\cup S_5$, the non trivial stages.
		\end{itemize}
		\item \label{item_P6_2}
		$\pst_\mathrm{pre}$ is also a $\lambda_4$-$\Lambda^\mathrm{lim}_\mathrm{cuf}$-iteration and has $\Lambda^\mathrm{lim}_\mathrm{cuf}$-limits on $H^\prime$ 
		with the following witnesses:
		\begin{itemize}
			\item $\langle\p_\xi^-:\xi<\gamma\rangle$, the (same as above) complete subposets witnessing $\Lambda^\mathrm{lim}_\mathrm{cuf}$-linkedness.
			\item $\bar{R}=\langle\dot{R}_{\xi,\zeta}:\zeta<\theta_\xi,\xi<\gamma\rangle$, the $\Lambda^\mathrm{lim}_\mathrm{cuf}$-linked components.
			\item $\langle \dot{E}^{h^\prime}_\xi:\xi\leq\gamma,~h^\prime\in H^\prime\rangle$, the ultrafilters.
			\item $T^-\coloneq S_1\cup S_2\cup S_3\cup S_4$, the trivial stages and $T^+\coloneq S_5$, the non-trivial stages.
		\end{itemize}
		\item 
		\label{item_N}
		%\footnote{These submodels have nothing to do with the submodels which shall be used in the separation of the right side.}
		For each $\xi<\gamma$, $N_\xi\preccurlyeq H_\Theta$ is a submodel where $\Theta$ is a sufficiently large regular cardinal satisfying:
		\begin{enumerate}
			\item $|N_\xi|<\lambda_{\ind(\xi)}$.
			\item \label{item_sigma_closed}
			% $N_\xi$ is closed under $\omega$-sequences 
			$N_\xi$ is $\sigma$-closed, i.e., $(N_\xi)^\omega\subseteq N_\xi$.
			
			\item 
			\label{item_N_e}For any $\ind\in I$, $\eta<\gamma$ and set of (nice names of) reals $A$ in $V^{\p_\eta}$ of size $<\lambda_\ind$,
			there is some $\xi\in S_\ind$ (above $\eta$) such that $A\subseteq N_\xi$.
			\item If $\ind(\xi)=4$, then $\{\dot{D}^h_\xi:h\in H \}\subseteq N_\xi$.
			\item If $\ind(\xi)=5$, then $\{\dot{D}^h_\xi:h\in H \},\{\dot{E}^{h^\prime}_\xi:h^\prime\in H^\prime \}\subseteq N_\xi$.
			
		\end{enumerate}
		
		\item $\p_\xi^-\coloneq\p_\xi\cap N_\xi$ (since $\p_\xi$ is ccc and $N_\xi$ is $\sigma$-closed, $\p_\xi^-\lessdot\p_\xi$).
		
		\item For each $\xi<\gamma$,
		$\p^-_\xi\Vdash\qd_\xi\coloneq\br_{\ind(\xi)}$. 
		
		(Here, $\br_{\ind(\xi)}$ does not denote a forcing poset in the ground model, but denotes the poset interpreted in the  $\p^-_\xi$-extension.
		Also note that $|\qd_\xi|<\lambda_{\ind(\xi)}$ holds since there are at most $|\p^-_\xi|^{\aleph_0}\leq|N_\xi|^{\aleph_0}<\lambda_{\ind(\xi)}$-many reals in the $\p^-_\xi$-extension.)
		\item $\bar{Q}$ and $\bar{R}$ are determined in the canonical way:
		In the case of $\bar{Q}$, if $\ind(\xi)=1,2,3$, split $\qd_\xi$ into singletons and if $\ind(\xi)=4,5$, split the $\sigma$-$\Lambda^\mathrm{lim}_\mathrm{uf}$-linked iterand $\qd_\xi$ into the $\omega$-many $\Lambda^\mathrm{lim}_\mathrm{uf}$-linked components. In the case of $\bar{R}$, do it similarly.
		
		
		
		%\item If $\xi\in S_\ind$, then $\Vdash_{\p_\xi}|\qd_\xi|<\lambda_\ind$.
		
		
	\end{enumerate}
	
	
	
	
\end{con}

%We explain why the construction is possible:

%\textit{Successor step.}
%At stage $\xi$, we can take some $N_\xi$ satisfying Construction \ref{con_P6}\eqref{item_N},
%by Assumption \ref{ass_card_arith}\eqref{item_aleph1_inacc} for Construction \ref{con_P6}\eqref{item_N}\eqref{item_sigma_closed} and by Assumption \ref{ass_card_arith} \eqref{item_ca_3} for Construction \ref{con_P6}\eqref{item_N}\eqref{item_N_e}, the bookkeeping condition.
%%We may also require that By Lemma \ref{lem_D_minus_in_suff},
%%$\Vdash_{\p_\xi}(\dot{D}^h_\xi)^-, (\dot{E}^{h^\prime}_\xi)^-\in V^{\p_\xi^-}$ for all $h\in H$ and $h^\prime\in H^\prime$.
%By Lemma \ref{lem_uf_const_succ}, Corollary \ref{cor_E_is_centered_suff_cuf} and Corollary \ref{cor_PR_is_sigma_centered_suff}, we obtain suitable $\{\dot{D}^h_{\xi+1}:h\in H \}$ and $\{\dot{E}^{h^\prime}_{\xi+1}:h^\prime\in H^\prime \}$: E.g., consider the most complicated case $\ind(\xi)=4$. On the one hand, since $\xi\in S^+$, $(\dot{D}^h_\xi)^-=\dot{D}^h_\xi\cap V^{\p_\xi^-}$ and $\dot{D}^h_\xi\in N_\xi$. Hence by Lemma \ref{lem_D_minus_in_suff}, $(\dot{D}^h_\xi)^-\in V^{\p^-_\xi}$ holds. On the other hand, since $\xi\in T^-$, $(\dot{E}^{h^\prime}_\xi)^-\in V^{\p^-_\xi}$ trivially holds.
%Thus, the assumption \eqref{eq_minus} is satisfied for both $\dot{D}^h_\xi$ and $\dot{E}^{h^\prime}_\xi$ and hence Lemma \ref{lem_uf_const_succ} can be applied. The other cases are similar and simpler: If $\ind(\xi)=1,2,3$, then $\xi$ is trivial for both $\bar{D}$ and $\bar{E}$. If $\ind(\xi)=5$, then $\xi$ is non-trivial for both, but $\{\dot{D}^h_\xi:h\in H \},\{\dot{E}^{h^\prime}_\xi:h^\prime\in H^\prime \}\subseteq N_\xi$. Hence, the assumption \eqref{eq_minus} is satisfied in any case. %Actually this is why we split trivial and nontrivial stages.)
%
%\textit{Limit step.}
%Direct from Lemma \ref{lem_uf_const_all}, \ref{lem_Ed_is_cuf} and \ref{lem_PR_uf}.


%To show that this construction can be done, it is enough to show that for each $\xi<\gamma$, if we have constructed all objects with index $\eta<\xi$, we can find $\langle\dot{D}_\xi^h:h\in H\rangle$, $\langle\dot{E}_\xi^h:h\in H\rangle$ and $N_\xi$, since $\langle\dot{Q}_{\xi,\zeta}:\zeta<\theta_\xi\rangle$ and $\langle\dot{R}_{\xi,\zeta}:\zeta<\theta_\xi\rangle$ are automatically determined. (In the case of $\langle\dot{Q}_{\xi,\zeta}:\zeta<\theta_\xi,\rangle$, if $\ind(\xi)=1,2,3$, split $\qd_\xi$ into singletons and if $\ind(\xi)=4,5$, split the $\sigma$-$\Lambda^\mathrm{lim}_\mathrm{uf}$-linked iterand $\qd_\xi$ into the $\omega$-many $\Lambda^\mathrm{lim}_\mathrm{uf}$-linked components. In the case of $\langle\dot{R}_{\xi,\zeta}:\zeta<\theta_\xi\rangle$, do it similarly.)
%
%For $\langle\dot{D}_\xi^h:h\in H\rangle$, 
%use Lemma \ref{lem_uf_const_all}, Corollary \ref{cor_E_is_centered_suff_cuf} and Corollary \ref{cor_PR_is_sigma_centered_suff}.
%
%For $\langle\dot{E}_\xi^h:h\in H\rangle$, 
%use Lemma \ref{lem_uf_const_all} and Corollary \ref{cor_E_is_centered_suff_cuf}.
%
%For $N_\xi$, use Assumption \ref{ass_card_arith}\eqref{item_aleph1_inacc} for Construction \ref{con_P6}\eqref{item_N}\eqref{item_sigma_closed} (and use bookkeeping argument for Construction \ref{con_P6}\eqref{item_N}\eqref{item_N_e}. Assumption \ref{ass_card_arith} \eqref{item_ca_3} enables the bookkeeping). 
%
%Thus, we can perform the iteration construction.

\begin{thm}
	\label{thm_p6_forces}
	$\pst_\mathrm{pre}$ forces for each $\ind\in I$,
	$\R_\ind\cong_T C_{[\lambda_6]^{<\lambda_\ind}}\cong_T[\lambda_6]^{<\lambda_\ind}$, in particular, $\bb(\R_\ind)=\lambda_\ind$ and $\dd(\R_\ind)=2^{\aleph_0}=\lambda_6$ (the same things also hold for $\R_4^*$).
	%(see Figure \ref{fig_left_of_CMe}).
\end{thm}

\begin{proof}
	
	Fact \ref{fac_Tukey_order_equivalence_condition} and Construction \ref{con_P6} \eqref{item_N}\eqref{item_N_e} imply $\R_\ind\lq C_{[\lambda_6]^{<\lambda_\ind}}$ for all $\ind\in I$.
	
	For $\ind=1,2$ and $5$, applying Corollary \ref{cor_smallness_for_addn_and_covn_and_nonm} with $\theta=\lambda_\ind$, 
	we obtain $C_{[\lambda_6]^{<\lambda_\ind}}\lq\R_\ind$.
	
	For $\ind=3$, Theorem \ref{thm_uf_limit_keeps_b_small} implies $C_{[\lambda_6]^{<\lambda_3}}\lq\R_3$.
	
	For $\ind=4$, Main Lemma \ref{lem_Main_Lemma} implies $C_{[\lambda_6]^{<\lambda_4}}\lq\R_4^*\lq\R_4$.
	
\end{proof}


%
%\begin{figure}
%	
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{1.5}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (l1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.2*\w, 0.7*\h) {$\lambda_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		\node (l2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.18*\w, 2.5*\h) {$\lambda_2$};
%		
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1*\h) {$\bb$};
%		\node (l3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.8*\w, 0.8*\h) {$\lambda_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		\node (l5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.35*\w, 3.35*\h) {$\lambda_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		
%		
%		\node[textnode] (d) at (\w*2,  2*\h) {$\dd$};
%		
%		
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		\node (l6) [fill=lime, draw, text=black, circle,inner sep=2.0pt] at (3.5*\w, 1.5*\h) {\scalebox{3.0}{$\lambda_6$}};%3.5 1.5 \Huge
%		
%		\node[textnode] (e) at (0.5*\w,  2*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  2*\h) {$\ee^*$};
%		\node (l4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.18*\w, 2.35*\h) {$\lambda_4$};
%		
%		\node[textnode] (pr) at (2.5*\w,  1*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1*\h) {$\mathfrak{pr}^*$};
%		
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (estar) to (d);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		
%		
%		\draw[blue,thick] (0.35*\w,2.6*\h)--(1.5*\w,2.6*\h);
%		\draw[blue,thick] (0.35*\w,1.5*\h)--(0.35*\w,2.6*\h);
%		
%		
%		\draw[blue,thick] (1.5*\w,-0.5*\h)--(1.5*\w,3.5*\h);
%		\draw[blue,thick] (0.5*\w,2.6*\h)--(0.5*\w,3.5*\h);
%		
%		
%		\draw[blue,thick] (0.5*\w,-0.5*\h)--(0.5*\w,1.5*\h);
%		
%		\draw[blue,thick] (-0.5*\w,-0.5*\h)--(-0.5*\w,3.5*\h);
%		\draw[blue,thick] (-0.5*\w,1.5*\h)--(1.5*\w,1.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Constellation of $\pst_\mathrm{pre}$ and $\pst_\mathrm{mid}$.}\label{fig_left_of_CMe}
%\end{figure}

\subsection{Recovery of GCH}
To apply the submodel method to separate the right side, we actually need some cardinal arithmetic (see \cite{GKMS}, \cite{forcing_constellations}), which is satisfied (particularly) under GCH, but \textit{conflicts} with Assumption \ref{ass_for_complete_guardrail}, which we have used for the completeness of the sets $H$ and $H^\prime$ of guardrails.
To avoid the conflict, we shall reconstruct the iteration under GCH. 
The argument of the reconstruction is as in \cite{GKS} and we obtain the following theorem.


\begin{thm}
	\label{thm_p6_GCH}
	Assume GCH and Assumption \ref{ass_card_arith}.
	Then, there exists a ccc poset $\pst_\mathrm{mid}$ which forces for each $\ind\in I$,
	$\R_\ind\cong_T C_{[\lambda_6]^{<\lambda_\ind}}\cong_T[\lambda_6]^{<\lambda_\ind}$, in particular, $\bb(\R_\ind)=\lambda_\ind$ and $\dd(\R_\ind)=2^{\aleph_0}=\lambda_6$ (the same things also hold for $\R_4^*$).
\end{thm}

\subsection{Separation of the right side}
Thanks to Theorem \ref{thm_p6_GCH}, we are now in the situation where the \textit{submodel method} can be applied, which was introduced in \cite{GKMS} and enables to separate the right side of the diagram.

%\begin{thm}
%	Assume GCH and 
%	$\aleph_1\leq\theta_1\leq\theta_2\leq\theta_3\leq\theta_4\leq\theta_5\leq\kappa_5\leq\kappa_4\leq\kappa_3\leq\kappa_2\leq\kappa_1$ are regular and $\kappa_\cc\geq\kappa_1$ satisfies $\kappa_\cc^{\aleph_0}=\kappa_\cc$.
%	Then, there exists a ccc poset $\p^{\mathrm{fin}}$ which forces $\bb(\R_\ind)=\theta_\ind$, $\dd(\R_\ind)=\kappa_\ind$ and $\cc=\kappa_\cc$.
%\end{thm}
\begin{thm}
	\label{thm_p6fin}
	Assume GCH and 
	$\aleph_1\leq\theta_1\leq\cdots\leq\theta_{10}$ are regular and $\theta_\cc$ is infinite cardinal such that $\theta_\cc\geq\theta_{10}$ and $\theta_\cc^{\aleph_0}=\theta_\cc$.
	Then, there exists a ccc poset $\pst_{\mathrm{fin}}$ which forces $\bb(\R_\ind)=\theta_\ind$ and $\dd(\R_\ind)=\theta_{11-\ind}$ for each $\ind\in I$ (the same things also hold for $\R_4^*$) and $\cc=\theta_\cc$. %(see Figure \ref{fig_right_of_CMe}).
\end{thm}

\begin{proof}
	See \cite{GKMS}.
\end{proof}


%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{1.5}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.2*\w, 0.7*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.18*\w, 2.5*\h) {$\theta_2$};
%		
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1*\h) {$\bb$};
%		\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.8*\w, 0.8*\h) {$\theta_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.35*\w, 3.35*\h) {$\theta_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		\node (t6) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.65*\w, -0.4*\h) {$\theta_6$};
%		
%		\node[textnode] (d) at (\w*2,  2*\h) {$\dd$};
%		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.2*\w, 2.2*\h) {$\theta_8$};
%		
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.82*\w, 0.5*\h) {$\theta_9$};
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.2*\w, 2.3*\h) {$\theta_{10}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		\node (tcc) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.65*\w, 3.5*\h) {$\theta_\cc$};
%		
%		\node[textnode] (e) at (0.5*\w,  2*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  2*\h) {$\ee^*$};
%		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.18*\w, 2.35*\h) {$\theta_4$};
%		
%		\node[textnode] (pr) at (2.5*\w,  1*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1*\h) {$\mathfrak{pr}^*$};
%		\node (t7) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.82*\w, 0.65*\h) {$\theta_7$};
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (estar) to (d);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		
%		
%		\draw[blue,thick] (1.5*\w,0.4*\h)--(2.65*\w,0.4*\h);
%		\draw[blue,thick] (2.65*\w,0.4*\h)--(2.65*\w,1.5*\h);
%		\draw[blue,thick] (-0.5*\w,1.5*\h)--(3.5*\w,1.5*\h);
%		\draw[blue,thick] (0.35*\w,2.6*\h)--(1.5*\w,2.6*\h);
%		\draw[blue,thick] (0.35*\w,1.5*\h)--(0.35*\w,2.6*\h);
%		
%		
%		\draw[blue,thick] (1.5*\w,-0.4*\h)--(1.5*\w,3.5*\h);
%		\draw[blue,thick] (0.5*\w,2.6*\h)--(0.5*\w,3.5*\h);
%		\draw[blue,thick] (2.5*\w,1.5*\h)--(2.5*\w,3.5*\h);
%		
%		
%		\draw[blue,thick] (0.5*\w,-0.4*\h)--(0.5*\w,1.5*\h);
%		\draw[blue,thick] (2.5*\w,-0.4*\h)--(2.5*\w,0.4*\h);
%		\draw[blue,thick] (-0.5*\w,-0.4*\h)--(-0.5*\w,3.5*\h);
%		\draw[blue,thick] (3.5*\w,-0.4*\h)--(3.5*\w,3.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Constellation of $\pst_\mathrm{fin}$.}\label{fig_right_of_CMe}
%\end{figure}

\subsection{Controlling $\ee_{ubd}$}
Toward the proof of Theorem C, where $g$-prediction (Definition \ref{dfn_variant}) is treated in the separation, let us consider $\ee_g$ for $g\in(\omega\setminus2)^\omega$.

\begin{dfn}
	$\R_5^g\coloneq\mathbf{PR}_g$ for $g\in(\omega\setminus2)^\omega$.
\end{dfn}
By Lemma \ref{lem_PR_uf}, the poset $\mathbb{PR}_g$, which increases $\ee_g$, is $\sigma$-c-uf-limit-linked.
Thus, performing an iteration where the $\sigma$-c-uf-limit-linked forcing $\mathbb{E}$ is replaced with $\mathbb{PR}_g$ and where $g$ runs through all $g\in(\omega\setminus2)^\omega$ by bookkeeping, we obtain the following:%\footnote{$\pst^\prime_\mathrm{mid}$ is the poset constructed after the recovery of GCH.}:

\begin{thm}(Corresponding to Theorem \ref{thm_p6_GCH}, the construction of $\pst_\mathrm{mid}$.)
	\label{thm_p_mid_prime_GCH}
	Assume GCH and Assumption \ref{ass_card_arith}.
	Then, there exists a ccc poset $\pst^\prime_\mathrm{mid}$ which forces for each $\ind\in I$,
	$\R_\ind\cong_T C_{[\lambda_6]^{<\lambda_\ind}}\cong_T[\lambda_6]^{<\lambda_\ind}$, in particular, $\bb(\R_\ind)=\lambda_\ind$ and $\dd(\R_\ind)=2^{\aleph_0}=\lambda_6$ (the same things also hold for $\R_4^*$ and $\R_5^g$ for $g\in(\omega\setminus2)^\omega$).
\end{thm}

\begin{thm}(Corresponding to Theorem \ref{thm_p6fin}, the construction of $\pst_\mathrm{fin}$.)
	\label{thm_p_fin_prime_GCH}
	Assume GCH and 
	$\aleph_1\leq\theta_1\leq\cdots\leq\theta_{10}$ are regular and $\theta_\cc$ is infinite cardinal such that $\theta_\cc\geq\theta_{10}$ and $\theta_\cc^{\aleph_0}=\theta_\cc$.
	Then, there exists a ccc poset $\pst_{\mathrm{fin}}$ which forces $\bb(\R_\ind)=\theta_\ind$ and $\dd(\R_\ind)=\theta_{11-\ind}$ for each $\ind\in I$ (the same things also hold for $\R_4^*$ and $\R_5^g$ for $g\in(\omega\setminus2)^\omega$) and $\cc=\theta_\cc$. %(see Figure \ref{fig_cm_prime}).
\end{thm}


%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{1.5}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.2*\w, 0.7*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.18*\w, 2.5*\h) {$\theta_2$};
%		
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1*\h) {$\bb$};
%		\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.8*\w, 0.8*\h) {$\theta_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.35*\w, 3.35*\h) {$\theta_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		\node (t6) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.65*\w, -0.4*\h) {$\theta_6$};
%		
%		\node[textnode] (d) at (\w*2,  2*\h) {$\dd$};
%		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.2*\w, 2.2*\h) {$\theta_8$};
%		
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.82*\w, 0.5*\h) {$\theta_9$};
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.2*\w, 2.3*\h) {$\theta_{10}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		\node (tcc) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.65*\w, 3.5*\h) {$\theta_\cc$};
%		
%		\node[textnode] (e) at (0.5*\w,  2*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  2*\h) {$\ee^*$};
%		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.18*\w, 2.35*\h) {$\theta_4$};
%		
%		\node[textnode] (pr) at (2.5*\w,  1*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1*\h) {$\mathfrak{pr}^*$};
%		\node (t7) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.82*\w, 0.65*\h) {$\theta_7$};
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (estar) to (d);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		
%		
%		\draw[blue,thick] (1.5*\w,0.4*\h)--(2.65*\w,0.4*\h);
%		\draw[blue,thick] (2.65*\w,0.4*\h)--(2.65*\w,1.5*\h);
%		\draw[blue,thick] (-0.5*\w,1.5*\h)--(3.5*\w,1.5*\h);
%		\draw[blue,thick] (0.35*\w,2.6*\h)--(1.5*\w,2.6*\h);
%		\draw[blue,thick] (0.35*\w,1.5*\h)--(0.35*\w,2.6*\h);
%		
%		
%		\draw[blue,thick] (1.5*\w,-0.4*\h)--(1.5*\w,3.5*\h);
%		\draw[blue,thick] (0.5*\w,2.6*\h)--(0.5*\w,3.5*\h);
%		\draw[blue,thick] (2.5*\w,1.5*\h)--(2.5*\w,3.5*\h);
%		
%		
%		\draw[blue,thick] (0.5*\w,-0.4*\h)--(0.5*\w,1.5*\h);
%		\draw[blue,thick] (2.5*\w,-0.4*\h)--(2.5*\w,0.4*\h);
%		\draw[blue,thick] (-0.5*\w,-0.4*\h)--(-0.5*\w,3.5*\h);
%		\draw[blue,thick] (3.5*\w,-0.4*\h)--(3.5*\w,3.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Constellation of $\pst_\mathrm{fin}$.}\label{fig_right_of_CMe}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\tikzset{
%			textnode/.style={text=black}, 
%		}
%		\tikzset{
%			edge/.style={color=black, thin, opacity=0.5}, 
%		}
%		\newcommand{\w}{2.4}
%		\newcommand{\h}{2.0}
%		
%		\node[textnode] (addN) at (0,  0) {$\addn$};
%		\node (t1) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (-0.2*\w, 0.8*\h) {$\theta_1$};
%		
%		\node[textnode] (covN) at (0,  \h*3) {$\covn$};
%		\node (t2) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.15*\w, 2.45*\h) {$\theta_2$};
%		
%		
%		\node[textnode] (addM) at (\w,  0) {$\cdot$};
%		\node[textnode] (b) at (\w,  1.3*\h) {$\bb$};
%		\node (t3) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.68*\w, 1.2*\h) {$\theta_3$};
%		
%		\node[textnode] (nonM) at (\w,  \h*3) {$\nonm$};
%		\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (1.0*\w, 3.3*\h) {$\theta_5$};
%		
%		\node[textnode] (covM) at (\w*2,  0) {$\covm$};
%		\node (t6) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.0*\w, -0.3*\h) {$\theta_6$};
%		
%		\node[textnode] (d) at (\w*2,  1.7*\h) {$\dd$};
%		\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.32*\w, 1.8*\h) {$\theta_{8}$};
%		\node[textnode] (cofM) at (\w*2,  \h*3) {$\cdot$};
%		
%		
%		\node[textnode] (nonN) at (\w*3,  0) {$\nonn$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.85*\w, 0.55*\h) {$\theta_{9}$};
%		
%		\node[textnode] (cofN) at (\w*3,  \h*3) {$\cofn$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.25*\w, 2.2*\h) {$\theta_{10}$};
%		
%		\node[textnode] (aleph1) at (-\w,  0) {$\aleph_1$};
%		\node[textnode] (c) at (\w*4,  \h*3) {$2^{\aleph_0}$};
%		\node (t10) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (3.67*\w, 3.4*\h) {$\theta_\cc$};
%		
%		\node[textnode] (e) at (0.5*\w,  1.7*\h) {$\mathfrak{e}$}; 
%		\node[textnode] (estar) at (\w,  1.7*\h) {$\ee^*$};
%		\node (t4) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.75*\w, 1.9*\h) {$\theta_4$};
%		
%		
%		\node[textnode] (pr) at (2.5*\w,  1.3*\h) {$\mathfrak{pr}$}; 
%		\node[textnode] (prstar) at (\w*2,  1.3*\h) {$\mathfrak{pr}^*$};
%		\node (t9) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.25*\w, 1.1*\h) {$\theta_7$};
%		
%		\node[textnode] (eubd) at (\w*0.75,  \h*2.45) {$\ee_{ubd}$};
%		%\node[textnode] (nonE) at (\w*0.75,  \h*2.55) {$\non(\mathcal{E})$};
%		%\node (t5) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (0.5*\w, 2.1*\h) {$\theta_5$};%0.5 2.1
%		
%		\node[textnode] (prubd) at (\w*2.25,  \h*0.55) {$\mathfrak{pr}_{ubd}$};
%		%\node[textnode] (covE) at (\w*2.25,  \h*0.45) {$\cov(\mathcal{E})$};
%		%\node (t8) [fill=lime, draw, text=black, circle,inner sep=1.0pt] at (2.47*\w, 0.9*\h) {$\theta_8$};
%		
%		
%		
%		
%		
%		
%		
%		\draw[->, edge] (addN) to (covN);
%		\draw[->, edge] (addN) to (addM);
%		\draw[->, edge] (covN) to (nonM);	
%		\draw[->, edge] (addM) to (b);
%		%\draw[->, edge] (b) to (nonM);
%		\draw[->, edge] (addM) to (covM);
%		\draw[->, edge] (nonM) to (cofM);
%		%\draw[->, edge] (covM) to (d);
%		\draw[->, edge] (d) to (cofM);
%		\draw[->, edge] (b) to (prstar);
%		\draw[->, edge] (covM) to (nonN);
%		\draw[->, edge] (cofM) to (cofN);
%		\draw[->, edge] (nonN) to (cofN);
%		\draw[->, edge] (aleph1) to (addN);
%		\draw[->, edge] (cofN) to (c);
%		
%		%\draw[->, edge] (e) to (nonM);
%		\draw[->, edge] (e) to (covM);
%		\draw[->, edge] (addN) to (e);
%		
%		\draw[->, edge] (covM) to (prstar);
%		\draw[->, edge] (covM) to (prubd);
%		\draw[->, edge] (nonM) to (pr);
%		\draw[->, edge] (covN) to (prubd);
%		\draw[->, edge] (pr) to (cofN);
%		
%		\draw[->, edge] (e) to (estar);
%		\draw[->, edge] (b) to (estar);C
%		\draw[->, edge] (estar) to (nonM);
%		\draw[->, edge] (eubd) to (nonN);
%		\draw[->, edge] (estar) to (d);
%		\draw[->, edge] (e) to (eubd);
%		
%		\draw[->, edge] (prstar) to (d);
%		\draw[->, edge] (prstar) to (pr);
%		
%		\draw[->, edge] (prstar) to (pr);
%		\draw[->, edge] (prubd) to (pr);
%		\draw[->, edge] (eubd) to (nonM);
%		%		\
%		%		
%		%		\draw[->, edge] (eubd) to (nonE);
%		%		\draw[->, edge] (addM) to (nonE);
%		%		\draw[->, edge] (nonE) to (nonM);
%		%		
%		%		\draw[->, edge] (covE) to (prubd);
%		%		\draw[->, edge] (covE) to (cofM);
%		%		\draw[->, edge] (covM) to (covE);
%		
%		\draw[blue,thick] (-0.5*\w,1.5*\h)--(3.5*\w,1.5*\h);
%		\draw[blue,thick] (1.5*\w,-0.5*\h)--(1.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (-0.5*\w,-0.5*\h)--(-0.5*\w,3.5*\h);
%		\draw[blue,thick] (3.5*\w,-0.5*\h)--(3.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (0.5*\w,-0.5*\h)--(0.5*\w,1.5*\h);
%		\draw[blue,thick] (2.5*\w,1.5*\h)--(2.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (0.3*\w,2.25*\h)--(1.5*\w,2.25*\h);
%		%\draw[blue,thick] (-0.3*\w,2.7*\h)--(1.5*\w,2.7*\h);
%		\draw[blue,thick] (0.3*\w,1.5*\h)--(0.3*\w,2.25*\h);
%		\draw[blue,thick] (0.5*\w,2.25*\h)--(0.5*\w,3.5*\h);
%		
%		\draw[blue,thick] (2.7*\w,0.8*\h)--(1.5*\w,0.8*\h);
%		%\draw[blue,thick] (3.1*\w,0.3*\h)--(1.5*\w,0.3*\h);
%		\draw[blue,thick] (2.7*\w,1.5*\h)--(2.7*\w,0.8*\h);
%		\draw[blue,thick] (2.5*\w,0.8*\h)--(2.5*\w,-0.5*\h);
%		
%		
%		
%		
%		
%		
%		
%		
%		
%		
%	\end{tikzpicture}
%	\caption{Constellation of $\p^\prime_\mathrm{fin}$.}\label{fig_cm_prime}
%\end{figure}
%
%


==> preamble.tex <==
\RequirePackage{plautopatch}
\RequirePackage[l2tabu, orthodox]{nag}
\usepackage{bxtexlogo}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{amssymb, amsmath,stmaryrd,mathrsfs,mathtools}
%\usepackage{cancel}
\usepackage{tikz,float}
\usepackage{tikz-cd}
\usepackage{amsthm}
\usepackage{enumerate}

%\usepackage[compat=1.1.0]{tikz-feynhand}
\usetikzlibrary{calc}
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage{graphicx}
\usepackage{xcolor}
%\usepackage{xcolor}
%\usepackage[dvipsnames]{xcolor}
%\everymath{\displaystyle}

\pagestyle{plain}

\theoremstyle{definition}
\newtheorem{thm}{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{exa}[thm]{Example}
\newtheorem{dfn}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{que}[thm]{Question}
\newtheorem{fac}[thm]{Fact}
\newtheorem{con}[thm]{Construction}
\newtheorem{ass}[thm]{Assumption}
\newtheorem{mainlem}[thm]{Main Lemma}
\newtheorem*{clm}{Claim}
\newtheorem*{clm1}{Claim1}
\newtheorem*{clm2}{Claim2}
\newtheorem{ques}{Question}
\newtheorem*{thmA}{Theorem A}
\newtheorem*{thmB}{Theorem B}
\newtheorem*{thmC}{Theorem C}
\newtheorem*{thmm}{Theorem}
\newtheorem*{acknowledgements}{Acknowledgements}

\newtheorem{conjecture}[thm]{Conjecture}

\numberwithin{thm}{section} 
\numberwithin{equation}{section} 

\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}

\newcommand{\p}{\mathbb{P}}
\newcommand{\q}{\mathbb{Q}}
\newcommand{\br}{\mathbb{R}}
\newcommand{\bs}{\mathbb{S}}
\newcommand{\co}{\mathbb{C}}
\newcommand{\mat}{\mathbb{M}}
\newcommand{\ult}{\mathscr{U}}
\newcommand{\amo}{\mathbb{A}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\qd}{\dot{\mathbb{Q}}}
\newcommand{\leqd}{\dot{\leq}_\mathbb{Q}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\oneqd}{\dot{\mathbbm{1}}_\mathbb{Q}}
\DeclareMathAlphabet{\mymathbb}{U}{BOONDOX-ds}{m}{n}
\newcommand{\zero}{\mymathbb{0}}

\newcommand{\oo}{{\omega}^\omega}
\newcommand{\ooo}{[{\omega}]^\omega}
\newcommand{\fin}{[\omega]^{<\omega}}
\newcommand{\seq}{\omega^{<\omega}}
\newcommand{\sq}{2^{<\omega}}

\newcommand{\on}{\mathpunct{\upharpoonright}}

\newcommand{\ad}{\mathfrak{a}}
\newcommand{\bb}{\mathfrak{b}}
\newcommand{\cc}{\mathfrak{c}}
\newcommand{\dd}{\mathfrak{d}}
\newcommand{\ee}{\mathfrak{e}}
\newcommand{\pre}{\mathfrak{pr}}
\newcommand{\hh}{\mathfrak{h}}
\newcommand{\mm}{\mathfrak{m}}
\newcommand{\pp}{\mathfrak{p}}
\newcommand{\rr}{\mathfrak{r}}
\newcommand{\spl}{\mathfrak{s}}
\newcommand{\uu}{\mathfrak{u}}
\newcommand{\homo}{\mathfrak{hom}}
\newcommand{\parti}{\mathfrak{par}}
\newcommand{\m}{\mathcal{M}}
\newcommand{\n}{\mathcal{N}}

\newcommand{\covm}{\text{cov}(\mathcal{M})}
\newcommand{\nonm}{\text{non}(\mathcal{M})}
\newcommand{\addm}{\text{add}(\mathcal{M})}
\newcommand{\cofm}{\text{cof}(\mathcal{M})}
\newcommand{\covn}{\text{cov}(\mathcal{N})}
\newcommand{\nonn}{\text{non}(\mathcal{N})}
\newcommand{\addn}{\text{add}(\mathcal{N})}
\newcommand{\cofn}{\text{cof}(\mathcal{N})}
\newcommand{\covi}{\text{cov}(I)}
\newcommand{\noni}{\text{non}(I)}
\newcommand{\addi}{\text{add}(I)}
\newcommand{\cofi}{\text{cof}(I)}

\newcommand{\ii}{\mathcal{I}}
\newcommand{\jj}{\mathcal{J}}

\DeclareMathOperator{\cob}{COB}
\DeclareMathOperator{\eub}{EUB}
\DeclareMathOperator{\lcu}{LCU}
\newcommand{\R}{\mathbf{R}}
\newcommand{\bfs}{\mathbf{S}}

\renewcommand{\lq}{\preceq_T}

\DeclareMathOperator{\dep}{Dp}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\cf}{cf}
\DeclareMathOperator{\limdir}{limdir}
\DeclareMathOperator{\tbc}{tbc}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\non}{non}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\cof}{cof}
\DeclareMathOperator{\cfi}{cf}



\newcommand{\eeb}{\mathfrak{e}^*}
\newcommand{\preb}{\mathfrak{pr}^*}

\newcommand{\pr}{\mathbb{PR}}
\newcommand{\ev}{\mathbb{E}}

\newcommand{\bpd}{\sqsubset^\mathrm{bp}}
\newcommand{\suff}{\Lambda^\mathrm{suff}}

\newcommand{\Ad}{\mathbb{S}}


\DeclareMathOperator{\loss}{loss}
\DeclareMathOperator{\trunk}{trunk}
\DeclareMathOperator{\dns}{d}
\DeclareMathOperator{\intt}{int}
\newcommand{\bari}{\bar{I}=\langle I_k\rangle_{k<\omega}}

\DeclareMathOperator{\stem}{stem}


